BER-Based Physical Layer Security with Finite Codelength: Combining Strong Converse and Error Amplification

A bit error rate (BER)-based physical layer security approach is proposed for finite blocklength. For secure communication in the sense of high BER, the information-theoretic strong converse is combined with cryptographic error amplification achieved by substitution permutation networks (SPNs) based on confusion and diffusion. For discrete memoryless channels (DMCs), an analytical framework is provided showing the tradeoffs among finite blocklength, maximum/minimum possible transmission rates, and BER requirements for the legitimate receiver and the eavesdropper. Also, the security gap is analytically studied for Gaussian channels and the concept is extended to other DMCs including binary symmetric channels (BSCs) and binary erasure channels (BECs). For fading channels, the transmit power is optimized to minimize the outage probability of the legitimate receiver subject to a BER threshold for the eavesdropper.

==> additional_A.tex <==
\clearpage
\newpage
\section{Security Gap for GI-AWGN when $R \rightarrow \infty$}

{\it Corollary 1:} When $0< {\cal P}_\err^{\bob,\Th} <1$ and $0<{\cal P}_\err^{\eve,\Th} < 1$, the security gap is asymptotically given by \beqa \lim_{n \rightarrow \infty} \Delta S &=& 0  \\   \lim_{R \rightarrow \infty}\Delta S &=& 10 \log_{10} \frac{ (1 + \breve \rho_\infty) \left( {\cal P}_\err^{\bob,\Th} \right)^{-\frac{1}{n \breve \rho_\infty}}  }{(1+\breve \rho'_\infty)\left(1- {\cal P}_\err^{\eve,\Th} \right)^{-\frac{1}{n \breve \rho'_\infty}} }  \eeqa
where \beqa \breve \rho_\infty &=& \frac{1}{2} \left( \ln u_\bob + \left((\ln u_\bob)^2 + 4 \ln u_\bob \right)^{\frac{1}{2}} \right) \\  \breve \rho'_\infty &=& \frac{1}{2} \left(\ln u_\eve - \left((\ln u_\eve)^2 + 4 \ln u_\eve \right)^{\frac{1}{2}} \right) \eeqa
where $u_\bob = ({\cal P}_\err^{\bob,\Th})^{- \frac{1}{n} }$ and $u_\eve = (1-{\cal P}_\err^{\eve,\Th})^{- \frac{1}{n} }$.

{\it Proof:} As $n \rightarrow \infty$, we have $\min_{0 < \rho \leq 1} g_\bob(\rho) \rightarrow  (e^R-1)$ and $\max_{-1 < \rho' <0} g_\bob(\rho) \rightarrow (e^R-1)$, and thus, $\Delta S \rightarrow 0$. Also,
\beqa \lim_{R \rightarrow \infty} \Delta S &=& 10 \log_{10} \left( \lim_{R \rightarrow \infty} \frac{\min_{0 < \rho \leq 1} g_\bob(\rho)} {\min_{-1 < \rho' < 0} g_\eve(\rho')} \right) \\ &=& 10 \log_{10} \left( \lim_{R \rightarrow \infty} \frac{ g_\bob(\breve \rho_\infty)}{g_\eve(\breve \rho'_\infty)} \right). \eeqa In the above,
\beqa \breve \rho_\infty &=& \arg \lim_{R \rightarrow \infty} \min_{0 < \rho \leq 1} g_\bob(\rho) \\ &\stackrel{(a)}{=}&{\rm sol}_{\rho} \left\{ \lim_{R \rightarrow \infty} \frac{\partial }{\partial \rho} g_\bob(\rho)=0 \right\}  \\ \breve \rho'_\infty &=& \arg \lim_{R \rightarrow \infty} \min_{-1 < \rho' < 0} g_\eve(\rho') \\ &\stackrel{(b)}{=}& {\rm sol}_{\rho'} \left\{ \lim_{R \rightarrow \infty} \frac{\partial }{\partial \rho'} g_\eve(\rho')=0 \right\} \eeqa where ${\rm sol}_\alpha \{ f(\alpha) =0 \}$ denotes the solution to $f(\alpha) =0$. Note that $(a)$ holds only when the solution to $\lim_{R \rightarrow \infty} \frac{\partial }{\partial \rho} g_\bob(\rho)=0$ exist and it is unique. The same for $(b)$.
From \beq \lim_{R \rightarrow \infty} \frac{\partial }{\partial \rho} g_\bob(\rho) =\lim_{R \rightarrow \infty} \left\{ u_\bob^{\frac{1}{\rho}} e^R-1 + (1+\rho) \left( -\frac{1}{\rho^2} u_\bob^{\frac{1}{\rho}} e^R \ln u_\bob -1 \right) \right\} = 0\eeq we have \beq  u_\bob^{\frac{1}{\rho}}  - (1+\rho) \frac{1}{\rho^2} u_\bob^{\frac{1}{\rho}} \ln u_\bob   = 0\eeq There exists a unique valid solution to $\lim_{R \rightarrow \infty} \frac{\partial }{\partial \rho} g_\bob(\rho)=0$ and it is given by $\breve \rho_\infty =\frac{1}{2} \left( \ln u_\bob + \left((\ln u_\bob)^2 + 4 \ln u_\bob \right)^{\frac{1}{2}}\right)$. In the same way, one can show that there exist a unique solution to $\lim_{R \rightarrow \infty} \frac{\partial }{\partial \rho'} g_\eve(\rho')=0$ and it is given by $\breve \rho'_\infty =\frac{1}{2} \left( \ln u_\eve - \left((\ln u_\eve)^2 + 4 \ln u_\eve \right)^{\frac{1}{2}} \right)$.

\hfill $\Box$

(Question:) The range of $\breve \rho_\infty$ and $\breve \rho'_\infty$ must be \beqa 0 < \breve \rho_\infty \leq 1 \\ -1 < \breve \rho'_\infty < 0 \eeqa

How can we ensure this???

\clearpage
\newpage
\section{Security Gap for BSC}

{\it Remark:} Although the security gap was originally considered only for AWGN channels, the concept can be extended to other channels such as BSC and BEC. Let $\delta_\bob$ denote the crossover and erasure probabilities for BSC and BEC, respectively, for Bob. For BEC, we have \beqa E_0^\bob(\rho,q_{\rm uni}(x),\delta_\bob) &=& -\ln \left[ 2^{-\rho} (1-\delta_\bob) +\delta_\bob \right] \\ E_0^\eve(\rho',q_{\rm uni}(x),\delta_\eve) &=& -\ln \left[ 2^{-\rho'} (1-\delta_\eve) +\delta_\eve \right]  \eeqa For BSC, we have \beqa E_0^\bob(\rho,q_{\rm uni}(x),\delta_\bob) &=& -\ln \left[ 2^{-\rho} \left( \delta_\bob^{\frac{1}{1+\rho}}+(1-\delta_\bob)^{\frac{1}{1+\rho}} \right)^{1+\rho} \right] \\ E_0^\eve(\rho',q_{\rm uni}(x),\delta_\eve) &=& -\ln \left[ 2^{-\rho'} \left( \delta_\eve^{\frac{1}{1+\rho'}}+(1-\delta_\eve)^{\frac{1}{1+\rho'}} \right)^{1+\rho'} \right] \eeqa

The BER bounds are given by \beqa P_\ber^{\bob,\up}(R,\rho, \delta_\bob) &=& 0.5 \exp \left( -n \left\{ E_0^\bob(\rho,q_{\rm uni}(x),\delta_\bob)-\rho R \right\} \right) \\ P_\ber^{\eve,\low}(R,\rho', \delta_\eve) &=& P_\ber^{\rm SPN, \low}(r,K)\cdot \left( 1- \exp \left( -n \left\{ E_0^\eve(\rho',q_{\rm uni}(x),\delta_\eve)-\rho' R  \right\} \right) \right) \eeqa

Then an upper-bound of the security gap can be defined as the difference between the two probabilities as follows:
\beqa && \Delta S_\up  :=  \delta_{\eve,\up}^{\min} - \delta_{\bob,\low}^{\max} \eeqa where $\delta_\bob^{\max}$ and $\delta_\eve^{\min}$ are determined by \beqa \delta_{\bob,\low}^{\max}= \max \delta_\bob {\rm ~~~subject ~ to ~~~}  P_\ber^{\bob, \low}(R,\breve \rho,\delta_\bob) \leq \calP_\ber^{\bob,\Th} \\ \delta_{\eve,\up}^{\min}= \min \delta_\eve  {\rm ~~~subject ~ to ~~~} P_\ber^{\eve, \up}(R,\breve \rho', \delta_\eve) \geq \calP_\ber^{\eve,\Th}  \eeqa
where $\breve \rho$ is optimal $\rho$ minimizing $P_\ber^{\bob,\up}(R, \rho,\delta_\bob)$ and $\breve \rho'$ is optimal $\rho'$ maximizing $P_\ber^{\eve,\low}(R, \rho',\delta_\eve)$.



{\it Theorem 2:} $\delta_\bob^{\max}$ and $\delta_\eve^{\min}$ are \beqa \delta_\bob^{\max}(\rho) &=&  (1-2^{-\rho})^{-1} \left\{ \left(\varepsilon_\ber^{\bob,\Th} \right)^{\frac{1}{n}} e^{-\rho R} - 2^{-\rho} \right\} \\ \delta_\eve^{\min}(\rho') &=&  (1-2^{-\rho'})^{-1} \left\{ \left(\varepsilon_\ber^{\eve,\Th} \right)^{\frac{1}{n}} e^{-\rho' R} - 2^{-\rho'} \right\}
\\ \tilde \rho &=&\arg \max_{0 < \rho \leq 1}  \delta_\bob^{\max} (\rho) \label{eq:optimization_rho_1} \\ \tilde \rho' &=& \arg \min_{-1< \rho' <0}  \delta_\eve^{\min} (\rho'). \label{eq:optimization_rho_prime_1}  \eeqa

(Question:) We didn't get reasonable numerical results???

\clearpage
\newpage
\section{Outage probability when ${\cal P}_\err^{\eve,\Th} \rightarrow 0$. }

When ${\cal P}_\err^{\eve,\Th} \rightarrow 0$ (that is, with $no$ the security condition), the maximum power $p_{\max}(\Gamma_\eve, \rho') \rightarrow \infty$. Therefore, the overall outage probability must decrease indefinitely with $p_\av/\sigma^2$ with no error floor, as in the conventional outage probability of Caire's paper.

In my approach, however, we still have a error floor even when ${\cal P}_\err^{\eve,\Th} \rightarrow 0$. Please see the figure. The reason is as follows. No matter what the value of ${\cal P}_\err^{\eve,\Th}$, the maximum power $p_{\max}(\Gamma_\eve, \rho')$ is upper-limited by $p_0$, where $C_\eve = \ln(1 + p_0)$, because we use Eve's error lower-bound equation, which is valid only when $R> C_\eve$. Overall, even when ${\cal P}_\err^{\eve,\Th} \rightarrow 0$, we still have an error floor.

In the numerical results, the error floor is independent of ${\cal P}_\err^{\eve,\Th}$.


\begin{figure}[h]
\begin{center}
\includegraphics[width=1.1\columnwidth]{figure/Additional/additional_1}
\caption{Overall outage probability floor}
\label{fig:additional_1}
\end{center}
\end{figure}


\begin{figure}[h]
\begin{center}
\includegraphics[width=0.7\columnwidth]{figure/Additional/additional_2}
\caption{Overall outage probability floor}
\label{fig:additional_2}
\end{center}
\end{figure}


\clearpage
\newpage
\section{Minimization of Bob's Average BER subject to Security Constraint}

In this subsection, another approach is considered to optimize the transmit power. Taking expectation over $\gamma_\bob$, we first define Bob's average BER upper-bound as follows: \beqa \bar P_\ber^{\bob,\up}(R):&=& \mathbb{E} \left[ P_\ber^{\bob,\up}(R, \rho(\gamma_\bob),\gamma_\bob) \right], ~~~0< \rho \leq 1 \\ &=& 0.5 \mathbb{E} \left[ \exp \left( -n  \left\{  -\ln \left( 1+ \frac{ p \gamma_\bob  }{ (1+\rho(\gamma_\bob))  } \right)^{-\rho(\gamma_\bob)}  - \rho(\gamma_\bob) R \right\} \right) \right]. \label{eq:avg Bob_BER_Gau}    \eeqa
The transmit power is optimized to minimize $\bar P_\ber^{\bob,\up}(R)$ subject to a security constraint constraining Eve's instantaneous BER to be greater than a threshold as follows:
\begin{subequations}
\beqa && \min_{p(\gamma_\bob, \gamma_\eve),0< \rho(\gamma_\bob) \leq 1,-1< \rho'(\gamma_\eve)<0} \bar P_\ber^{\bob,\up}(R) \\ && {\rm subject ~ to} ~   p(\gamma_\bob, \gamma_\eve) \geq 0\\ && \hspace{1.9cm} \mathbb{E}[p(\gamma_\bob, \gamma_\eve)] \leq p_\av \\ && \hspace{1.9cm}  P_\ber^{\eve,\low}(R,\rho'(\gamma_\eve),\gamma_\eve) \geq \calP_\ber^{\eve,\Th}.\label{eq:prob_2_opt_1_constraint_3}  \eeqa \label{eq:prob_2_opt_1}   \end{subequations}
In the following, the optimal solution is derived.

{\it Theorem 2:} The optimal solution to (\ref{eq:prob_2_opt_1}) is given by
\beq p_{\opt 2}(\gamma_\bob, \gamma_\eve) = \min \left(p_\opt^{\bob,\up}(\gamma_\bob,\hat \rho,\lambda), p_{\max}(\gamma_\eve,\tilde \rho')  \right) \label{eq:p_opt2} \eeq
where $p_{\max}(\gamma_\eve, \rho')$ is given by (\ref{eq:p_max_Eve}) and   $p_\opt^{\bob,\up}(\gamma_\bob,\rho,\lambda)$ is given by
\beq p_\opt^{\bob,\up}(\gamma_\bob,\rho,\lambda) = \left( \left(\frac{\lambda \gamma_\bob^{\rho}}{ \rho (1+  \rho)^{  \rho} }\right)^{-\frac{1}{  \rho+1}} - \frac{1+ \rho}{\gamma_\bob} \right)^+. \label{eq:p_opt_b_u} \eeq
In (\ref{eq:p_opt2}), $\tilde \rho'$ is determined by (\ref{eq:optimization_rho_prime_1}) and then $\hat \rho(\gamma_\bob)$ is determined by
\beqa \hat \rho(\gamma_\bob) &=& \arg \max_{0<\rho(\gamma_\bob) \leq 1}  \left\{ E_0^\bob \left(\rho(\gamma_\bob),{\cal CN}\left(0,\min\left(p_\opt^{\bob,\up}(\gamma_\bob,\rho (\gamma_\bob),\lambda), p_{\max}(\gamma_\eve,\tilde \rho')  \right) \right),\gamma_\bob\right) - \rho(\gamma_\bob) R \right\} \non \\
\\ &=& \arg \max_{0<\rho(\gamma_\bob) \leq 1}  \left\{ -\ln \left( 1+ \frac{ \min \left(p_\opt^{\bob,\up}(\gamma_\bob, \rho(\gamma_\bob),\lambda), p_{\max}(\gamma_\eve, \tilde \rho')  \right) \gamma_\bob  }{1+\rho(\gamma_\bob)} \right)^{-\rho(\gamma_\bob)} - \rho(\gamma_\bob) R \right\} \non \\ \label{eq:optimizatio_hat_rho} \eeqa where the optimal $\hat \rho(\gamma_\bob)$ always exists and $\lambda$ is determined such that the following condition is satisfied:\beqa \mathbb{E} [  p_{\opt 2}(\gamma_\bob, \gamma_\eve)]= p_\av . \eeqa

{\it Proof of Theorem 2:} See Appendix B. \hfill $\Box$

Note that the exponent is positive: \beq E_0^\bob \left(\hat\rho(\gamma_\bob),{\cal CN}\left(0,p_{\opt 2}( \gamma_\bob,\gamma_\eve)  \right),\gamma_\bob\right) - \hat \rho(\gamma_\bob) R>0, ~~~~ R< C_\bob(\gamma_\bob,\gamma_\eve) \eeq where $C_\bob(\gamma_\bob,\gamma_\eve)$ is time-varying given by \beq C_\bob(\gamma_\bob,\gamma_\eve) = \ln \left(1+ \min \left(p_\opt^{\bob,\up}(\gamma_\bob,\hat \rho,\lambda), p_{\max}(\gamma_\eve,\tilde \rho')\right) \gamma_\bob \right) \eeq

(Problem): Depending on $\gamma_\bob$ and $\gamma_\eve$, the following situation happens \beq R > C_\bob(\gamma_\bob, \gamma_\eve) \eeq In this case, $E_0^\bob(\cdot) < 0$ and the corresponding instantaneous BER is 0.5, which makes the average BER not very small even when all other instantaneous BERs are extremely small.

In particular, when $p_\av \rightarrow \infty$, we have $p_\opt^{\bob,\up}(\gamma_\bob,\hat \rho,\lambda) \rightarrow \infty$; but $p_{\max}(\cdot)$ is not affected by $p_\av$. Therefore, the capacity is bounded by $p_{\max}(\cdot)$: \beqa C_\bob(\gamma_\bob, \gamma_\eve) & \leq & \ln \left(1+  p_{\max}(\gamma_\eve,\tilde \rho') \gamma_\bob \right) \\ & =: & C'_\bob(\gamma_\bob,\gamma_\eve) \eeqa Note that $C'_\bob(\gamma_\bob,\gamma_\eve)$ is time-varying and it is very possible: \beq R > C'_\bob(\gamma_\bob, \gamma_\eve) \eeq

\newpage

We now assume that $\rho$ is a constant that is independent of $\gamma_\bob$. Taking expectation over $\gamma_\bob$, we first define Bob's average BER upper-bound as follows: \beqa \hat P_\ber^{\bob,\up}(R,\rho):&=& \mathbb{E} \left[ P_\ber^{\bob,\up}(R, \rho,\gamma_\bob) \right], ~~~0< \rho \leq 1 \\ &=& 0.5 \exp \left( -n  \left\{  -\ln \mathbb{E} \left[ \left( 1+ \frac{ p \gamma_\bob  }{ (1+\rho)  } \right)^{-\rho} \right] - \rho R \right\} \right) . \label{eq:avg Bob_BER_Gau}    \eeqa
The transmit power is optimized to minimize $\bar P_\ber^{\bob,\up}(R,\rho)$ subject to a security constraint constraining Eve's instantaneous BER to be greater than a threshold as follows:
\begin{subequations}
\beqa && \min_{p(\gamma_\bob, \gamma_\eve),0< \rho \leq 1,-1< \rho'<0} \hat P_\ber^{\bob,\up}(R,\rho) \\ && {\rm subject ~ to} ~   p(\gamma_\bob, \gamma_\eve) \geq 0\\ && \hspace{1.9cm} \mathbb{E}[p(\gamma_\bob, \gamma_\eve)] \leq p_\av \\ && \hspace{1.9cm}  P_\ber^{\eve,\low}(R,\rho',\gamma_\eve) \geq \calP_\ber^{\eve,\Th}.\label{eq:prob_2_opt_1_constraint_3}  \eeqa \label{eq:prob_2_opt_1}   \end{subequations}
In the following, the optimal solution is derived.

{\it Corollary 2:} The optimal solution to (\ref{eq:prob_2_opt_1}) is given by
\beq p_{\opt 2}(\gamma_\bob, \gamma_\eve) = \min \left(p_\opt^{\bob,\up}(\gamma_\bob,\hat \rho,\lambda), p_{\max}(\gamma_\eve,\tilde \rho')  \right) \label{eq:p_opt2} \eeq
where $p_{\max}(\gamma_\eve, \rho')$ is given by (\ref{eq:p_max_Eve}) and   $p_\opt^{\bob,\up}(\gamma_\bob,\rho,\lambda)$ is given by
\beq p_\opt^{\bob,\up}(\gamma_\bob,\rho,\lambda) = \left( \left(\frac{\lambda \gamma_\bob^{\rho}}{ \rho (1+  \rho)^{  \rho} }\right)^{-\frac{1}{  \rho+1}} - \frac{1+ \rho}{\gamma_\bob} \right)^+. \label{eq:p_opt_b_u} \eeq
In (\ref{eq:p_opt2}), $\tilde \rho'$ is determined by (\ref{eq:optimization_rho_prime_1}) and then $\hat \rho$ is determined by
\beqa \hat \rho &=&\arg \max_{0<\rho \leq 1}  \left( -\ln \mathbb{E} \left[ \left( 1+ \frac{ \min \left(p_\opt^{\bob,\up}(\gamma_\bob, \rho,\lambda), p_{\max}(\gamma_\eve, \tilde \rho')  \right) \gamma_\bob  }{1+\rho} \right)^{-\rho}\right] - \rho R \right) \label{eq:optimizatio_hat_rho} \eeqa where the optimal $\hat \rho$ always exists and $\lambda$ is determined such that the following condition is satisfied:\beqa \mathbb{E} [  p_{\opt 2}(\gamma_\bob, \gamma_\eve)]= p_\av . \eeqa Finally, with $p_{\opt 2}(\gamma_\bob, \gamma_\eve)$, the exponent in (\ref{eq:avg Bob_BER_Gau}) is positive: \beq -\ln \mathbb{E} \left[ \left( 1+ \frac{ p_{\opt 2}(\gamma_\bob,\gamma_\eve) \gamma_\bob  }{ (1+\hat \rho)  } \right)^{-\hat \rho} \right] - \hat \rho R>0, ~~~~ R <C_\bob. \eeq

{\it Proof of Theorem 2:} See Appendix B. \hfill $\Box$

The result of Theorem 2 can be explained as follows. If the security condition of (\ref{eq:prob_2_opt_1_constraint_3}) is {\it not} imposed, $p_\opt^{\bob,\up}(\gamma_\bob, \rho,\lambda)$ is the optimal solution to (\ref{eq:prob_2_opt_1}), which can be obtained by the Lagrangian method. Also, $p_{\max}(\gamma_\eve,\tilde \rho')$ is the maximum allowable power to avoid any security outage as discussed in Theorem 1. Therefore, the optimum power $p_{\opt 2}(\gamma_\bob,\gamma_\eve)$ must be upper-limited by $p_{\max}(\gamma_\eve,\tilde \rho')$, because the security condition of (\ref{eq:prob_2_opt_1_constraint_3}) cannot be satisfied with higher power. Overall, the the optimum power $p_{\opt 2}(\gamma_\bob,\gamma_\eve)$ is given by the minimum of $p_\opt^{\bob,\up}(\gamma_\bob, \rho,\lambda)$ and $p_{\max}(\gamma_\eve,\tilde \rho')$. Finally, $\rho$ is optimized to minimize $\bar P_\ber^{\bob,\up}(R,\rho)$ as in (\ref{eq:optimizatio_hat_rho}).

{\it Remark 5:} If we compare the two problems of (\ref{eq:prob_1_opt_1}) and (\ref{eq:prob_2_opt_1}), the security condition is instantaneously satisfied for both problems. However, the achieved BER at Bob is different for the two problems. With the optimal power allocation of Theorem 2, Bob's instantaneous BER can be higher (or lower) than the average BER upper-bound, because only the average BER upper-bound is minimized. This is in sharp contrast to the first power optimization of Theorem 1, where the data transmission is suspended if Bob's instantaneous BER is higher than a threshold, which means that Bob's instantaneous BER is guaranteed to be always higher than the threshold whenever the data is transmitted.

\subsection{numerical results}

We now evaluate Bob's average BER upper-bound $\bar P_\ber^{\bob, \up}(R, \hat \rho)$ of (\ref{eq:avg Bob_BER_Gau}) with optimal $\hat \rho$. Rate $R$ is set to 2 and the security condition is given by $\varepsilon_\ber^{\eve,\Th}=10^{-4}$. Three different blocklengths are considered: $n \in \{500, 10^3, 10^4\}$. Applying the optimal power allocation of Theorem 2, the achieved minimum $\bar P_\ber^{\bob, \up}(R, \hat \rho)$ is presented in Fig. \ref{fig:BER_minimization_opt}. As can be expected, with more power $p_{\rm av}$ or longer blocklength $n$, Bob's average BER upper-bound improves.


%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=0.7\columnwidth]{figure/BER_minimization_opt}
%\caption{Bob's average BER upper-bound $\bar P_\ber^{\bob, \up}(R, \hat \rho)$ obtained by the optimal power allocation of Theorem 2. $\varepsilon_\ber^{\eve,\Th}=10^{-4}$. $\mathbb{E}[|h_\bob|^2]=2$ and $\mathbb{E}[|h_\eve|^2]=1$. $R=2$.}
%\label{fig:BER_minimization_opt}
%\end{center}
%\end{figure}


\clearpage \newpage

\section*{Appendix A\\Proof of Theorem 2}
\renewcommand\theequation{A.\arabic{equation}}
\setcounter{equation}{0}

The problem of (\ref{eq:prob_2_opt_1}) can be rewritten as \begin{subequations} \beqa &&  \min_{0< \rho(\gamma_\bob) \leq 1, -1<\rho'(\gamma_\eve) <0} \min_{p(\gamma_\bob,\gamma_\eve,\rho(\gamma_\bob),\rho'(\gamma_\eve))} \bar P_\ber^{\bob,\up}(R) \\ && {\rm subject ~ to} ~   p(\gamma_\bob,\gamma_\eve,\rho(\gamma_\bob),\rho'(\gamma_\eve)) \geq 0\\ && \hspace{1.9cm} \mathbb{E}[p(\gamma_\bob,\gamma_\eve,\rho(\gamma_\bob),\rho'(\gamma_\eve))] \leq p_\av   \\ &&  \hspace{1.9cm}   p(\gamma_\bob,\gamma_\eve,\rho(\gamma_\bob),\rho'(\gamma_\eve)) \leq p_{\max}(\gamma_\eve,\rho') \label{eq:equivalent_optimization_2_constraint_3}   \eeqa \end{subequations}
where (\ref{eq:equivalent_optimization_2_constraint_3}) is obtained by substituting $P_\ber^{\eve,\low}(R,\rho'(\gamma_\eve),\gamma_\eve)$ of (\ref{eq:Eve_BER_Gau}) into (\ref{eq:prob_2_opt_1_constraint_3}) and $p_{\max}(\gamma_\eve,\rho')$ is given by (\ref{eq:p_max_Eve}). Using the Lagrangian multiplier, it is possible to derive the optimal solution given by \beq p_{\opt 2}(\gamma_\bob,\gamma_\eve,\rho(\gamma_\bob),\rho'(\gamma_\eve)) = \min \left(   \left( \left(\frac{\lambda \gamma_\bob^{\rho(\gamma_\bob)}}{\rho(\gamma_\bob) (1+ \rho(\gamma_\bob))^{ \rho(\gamma_\bob)} }\right)^{-\frac{1}{ \rho(\gamma_\bob)+1}} - \frac{1+\rho(\gamma_\bob)}{\gamma_\bob} \right)^+, p_{\max}(\gamma_\eve, \rho') \right) \eeq
where
$\lambda$ is determined such that the average power constraint is satisfied:
\beqa \mathbb{E} [  p_{\opt 2}(\gamma_\bob,\gamma_\eve,\rho(\gamma_\bob), \rho'(\gamma_\eve))]= p_\av.  \eeqa

We now optimize $\rho(\gamma_\bob)$ and $\rho'(\gamma_\eve)$ to minimize $\bar P_\ber^{\bob,\up}(R)$ with $p_{\opt 2}(\gamma_\bob,\gamma_\eve,\rho(\gamma_\bob),\rho'(\gamma_\eve))$ as follows:
\beqa && (\hat \rho(\gamma_\bob), \hat \rho'(\gamma_\eve)) \non \\ &=& \arg \min_{0<\rho(\gamma_\bob) \leq 1,-1< \rho'(\gamma_\eve)<0} \left.
\bar P_\ber^{\bob,\up}(R) \right|_{p=p_{\opt 2}(\gamma_\bob,\gamma_\eve, \rho(\gamma_\bob),\rho'(\gamma_\eve))}\\
&=&\arg \max_{0<\rho(\gamma_\bob) \leq 1,-1< \rho'(\gamma_\eve)<0}  \left( -\ln \left( 1+ \frac{ \min \left( p_\opt^{\bob,\up}(\gamma_\bob,\rho(\gamma_\bob),\lambda), p_{\max}(\gamma_\eve,\rho') \right) \gamma_\bob  }{1+\rho(\gamma_\bob)} \right)^{-\rho(\gamma_\bob)} - \rho(\gamma_\bob) R \right) \non \\ \\ &=&\arg \max_{0<\rho(\gamma_\bob) \leq 1}  \left( -\ln \left( 1+ \frac{ \min \left( p_\opt^{\bob,\up}(\gamma_\bob,\rho(\gamma_\bob),\lambda), \max_{-1 <\rho' <0} p_{\max}(\gamma_\eve,\rho') \right) \gamma_\bob  }{1+\rho(\gamma_\bob)  } \right)^{-\rho(\gamma_\bob)} - \rho(\gamma_\bob) R \right). \non \\ \eeqa
The optimal $\hat \rho'$ is first obtained by
\beqa \hat \rho' &=& \arg \max_{-1< \rho' <0} p_{\max}(\gamma_\eve,\rho') \\ &=& \tilde \rho'. \eeqa
Then optimal $\hat \rho(\gamma_\bob)$ is obtained by minimizing $\bar P_\ber^{\bob,\up}(R)$: \beqa \hat \rho(\gamma_\bob) &=& \arg \max_{0 < \rho(\gamma_\bob) \leq 1} \left\{ -\ln  \left( 1+ \frac{ p_{\opt 2} (\gamma_\bob,\gamma_\eve,\rho(\gamma_\bob), \tilde \rho') \gamma_\bob  }{1+\rho(\gamma_\bob)} \right)^{-\rho(\gamma_\bob)}- \rho(\gamma_\bob) R  \right\}. \label{eq:appendix_B_hat_rho} \eeqa

Finally, to show the existence of the optimal solution $\hat \rho(\gamma_\bob)$, we rewrite the term $-\ln (\cdot)$ in (\ref{eq:appendix_B_hat_rho}) as follows: \beqa -\ln  \left( 1+ \frac{ p_{\opt 2}(\gamma_\bob,\gamma_\eve,\rho, \tilde \rho') \gamma_\bob  }{1+\rho} \right)^{-\rho} &=& -\ln   \int_{y_\bob} \left[ \int_x q_{\cal CN}(x) f(y_\bob|x, h_\bob)^{\frac{1}{1+\rho}}   dx \right]^{1+\rho} dy_\bob \non \\ \\ &=:&  E_0^\bob(\rho, q_{\cal CN}(x)) \eeqa where $q_{\cal CN}(x) ={\cal CN}(0,p_\opt(\gamma_\bob,\gamma_\eve,\rho, \breve \rho'))$ and $f(y_\bob|x, h_\bob)$ is given by (\ref{eq:bob_transition_Gau}).
Following the proof of \cite[Theorem 5.6.3 ]{gallager}, it can be shown that, with $\rho >0$, we have $\bar E_0^\bob(\rho,q(x)) > 0$, $\frac{\partial}{\partial \rho}\bar E_0^\bob(\rho,q(x)) > 0$, and $\frac{\partial^2}{\partial \rho^2}\bar E_0^\bob(\rho,q(x)) \leq 0$ for $R< C_\bob$ and for any $q(x)$. The cost function $\{-\ln \mathbb{E}[\cdot]-\rho R\}$ in (\ref{eq:appendix_B_hat_rho}) is the difference between a convex function and a straight line; and thus, the cost function is convex too. Based on the proof of \cite[Theorem 5.6.3 ]{gallager}, for $R<C_\bob$ and for any $q(x)$, it can be shown that optimal $\hat \rho$ exists in $(0,1]$ and the achieved maximum value is positive: \beq \max_{0 < \rho \leq 1} \left\{ \bar E_0^\bob(\rho,q(x)) -\rho R \right\} >0, ~~~~{\rm for~} R< C_\bob {\rm ~ and ~for ~ any~} q(x). \eeq




\clearpage \newpage

\section*{Appendix B\\Proof of Corollary 2}
\renewcommand\theequation{B.\arabic{equation}}
\setcounter{equation}{0}

The problem of (\ref{eq:prob_2_opt_1}) can be rewritten as \begin{subequations} \beqa &&  \min_{0< \rho \leq 1, -1<\rho' <0} \min_{p(\gamma_\bob,\gamma_\eve,\rho,\rho')} \bar P_\ber^{\bob,\up}(R,\rho) \\ && {\rm subject ~ to} ~   p(\gamma_\bob,\gamma_\eve,\rho,\rho') \geq 0\\ && \hspace{1.9cm} \mathbb{E}[p(\gamma_\bob,\gamma_\eve,\rho,\rho')] \leq p_\av   \\ &&  \hspace{1.9cm}   p(\gamma_\bob,\gamma_\eve,\rho,\rho') \leq p_{\max}(\gamma_\eve,\rho') \label{eq:equivalent_optimization_2_constraint_3}   \eeqa \end{subequations}
where (\ref{eq:equivalent_optimization_2_constraint_3}) is obtained by substituting $P_\ber^{\eve,\low}(R,\rho',\gamma_\eve)$ of (\ref{eq:Eve_BER_Gau}) into (\ref{eq:prob_2_opt_1_constraint_3}) and $p_{\max}(\gamma_\eve,\rho')$ is given by (\ref{eq:p_max_Eve}). Using the Lagrangian multiplier, it is possible to derive the optimal solution given by \beq p_{\opt 2}(\gamma_\bob,\gamma_\eve,\rho,\rho') = \min \left(   \left( \left(\frac{\lambda \gamma_\bob^{\rho}}{\rho (1+ \rho)^{ \rho} }\right)^{-\frac{1}{ \rho+1}} - \frac{1+\rho}{\gamma_\bob} \right)^+, p_{\max}(\gamma_\eve, \rho') \right) \eeq
where
$\lambda$ is determined such that the average power constraint is satisfied:
\beqa \mathbb{E} [  p_{\opt 2}(\gamma_\bob,\gamma_\eve,\rho, \rho')]= p_\av.  \eeqa

We now optimize $\rho$ and $\rho'$ to minimize $\bar P_\ber^{\bob,\up}(R,\rho)$ with $p_{\opt 2}(\gamma_\bob,\gamma_\eve,\rho,\rho')$ as follows:
\beqa && (\hat \rho, \hat \rho') \non \\ &=& \arg \min_{0<\rho \leq 1,-1< \rho'<0} \left.
\bar P_\ber^{\bob,\up}(R) \right|_{p=p_{\opt 2}(\gamma_\bob,\gamma_\eve, \rho,\rho')}\\
&=&\arg \max_{0<\rho \leq 1,-1< \rho'<0}  \left( -\ln \mathbb{E} \left[ \left( 1+ \frac{ \min \left( p_\opt^{\bob,\up}(\gamma_\bob,\rho,\lambda), p_{\max}(\gamma_\eve,\rho') \right) \gamma_\bob  }{1+\rho} \right)^{-\rho}\right] - \rho R \right) \non \\ \\ &=&\arg \max_{0<\rho \leq 1}  \left( -\ln \mathbb{E} \left[ \left( 1+ \frac{ \min \left( p_\opt^{\bob,\up}(\gamma_\bob,\rho,\lambda), \max_{-1 <\rho' <0} p_{\max}(\gamma_\eve,\rho') \right) \gamma_\bob  }{1+\rho  } \right)^{-\rho}\right] - \rho R \right). \non \\ \eeqa
The optimal $\hat \rho'$ is first obtained by
\beqa \hat \rho' &=& \arg \max_{-1< \rho' <0} p_{\max}(\gamma_\eve,\rho') \\ &=& \tilde \rho'. \eeqa
Then optimal $\hat \rho$ is obtained by minimizing $\bar P_\ber^{\bob,\up}(R)$: \beqa \hat \rho &=& \arg \max_{0 < \rho \leq 1} \left\{ -\ln \mathbb{E} \left[ \left( 1+ \frac{ p_{\opt 2} (\gamma_\bob,\gamma_\eve,\rho, \tilde \rho') \gamma_\bob  }{1+\rho} \right)^{-\rho}\right]- \rho R  \right\}. \label{eq:appendix_B_hat_rho} \eeqa

Finally, to show the existence of the optimal solution $\hat \rho$, we rewrite the term $-\ln \mathbb{E}[\cdot]$ in (\ref{eq:appendix_B_hat_rho}) as follows: \beqa -\ln \mathbb{E} \left[ \left( 1+ \frac{ p_{\opt 2}(\gamma_\bob,\gamma_\eve,\rho, \tilde \rho') \gamma_\bob  }{1+\rho} \right)^{-\rho}\right] &=& -\ln \mathbb{E}\left[  \int_{y_\bob} \left[ \int_x q_{\cal CN}(x) f(y_\bob|x, h_\bob)^{\frac{1}{1+\rho}}   dx \right]^{1+\rho} dy_\bob \right]\non \\ \\ &=:& \bar E_0^\bob(\rho, q_{\cal CN}(x)) \eeqa where $q_{\cal CN}(x) ={\cal CN}(0,p_\opt(\gamma_\bob,\gamma_\eve,\rho, \breve \rho'))$ and $f(y_\bob|x, h_\bob)$ is given by (\ref{eq:bob_transition_Gau}).
Following the proof of \cite[Theorem 5.6.3 ]{gallager}, it can be shown that, with $\rho >0$, we have $\bar E_0^\bob(\rho,q(x)) > 0$, $\frac{\partial}{\partial \rho}\bar E_0^\bob(\rho,q(x)) > 0$, and $\frac{\partial^2}{\partial \rho^2}\bar E_0^\bob(\rho,q(x)) \leq 0$ for $R< C_\bob$ and for any $q(x)$. The cost function $\{-\ln \mathbb{E}[\cdot]-\rho R\}$ in (\ref{eq:appendix_B_hat_rho}) is the difference between a convex function and a straight line; and thus, the cost function is convex too. Based on the proof of \cite[Theorem 5.6.3 ]{gallager}, for $R<C_\bob$ and for any $q(x)$, it can be shown that optimal $\hat \rho$ exists in $(0,1]$ and the achieved maximum value is positive: \beq \max_{0 < \rho \leq 1} \left\{ \bar E_0^\bob(\rho,q(x)) -\rho R \right\} >0, ~~~~{\rm for~} R< C_\bob {\rm ~ and ~for ~ any~} q(x). \eeq


{\it Temp 1:} Take expectation $\mathbb{E}[\cdot]$ to both sides of \cite[eq. (5B.11)]{gallager} and then take logarithm as in eq. (5B.12).


{\it Temp 2:}Following the approach \cite{Arimoto}, \cite[Lemma 3.2.1]{viterbi}, it can be shown that, with $-1< \rho' <0$, we have $\bar E_0^\eve(\rho',q(x)) < 0$, $\frac{\partial}{\partial \rho'}\bar E_0^\eve(\rho',q(x)) > 0$, and $\frac{\partial^2}{\partial \rho'^2}\bar E_0^\eve(\rho',q(x)) \leq 0$ for $R> C_\eve$ and any $q(x)$. Then it can be shown that optimal $\tilde \rho'$ exists in $(-1,0)$ and the achieved maximum value is positive as follows: \beqa 0 & < & \max_{-1 < \rho' <0} \left\{ \min_{q(x)} \bar E_0^\eve(\rho',q(x)) -\rho' R \right\} , ~~~~ R >  C_\eve \\ & \leq & \max_{-1 < \rho' <0} \left\{  \bar E_0^\eve(\rho',q_{\cal CN}(x)) -\rho' R \right\} , ~~~~ R >  C_\eve \eeqa where the inequality is due to \cite{Arimoto}, \cite[Theorem 3.9.1]{viterbi}.




























































%%%












==> comparison_achievability_converse.tex <==
\clearpage
\newpage

\begin{center}
{\bf \Large Comparisons of Proofs of Achievability and Strong Converse}

\vspace{0.5cm}
Il-Min Kim

April 22, 2014

\vspace{1cm}
\end{center}

Consider a code composed of $M=e^{nR}$ signal vectors (or codewords) $\bfx_m, m=1,\cdots,M$ of length $n$, whose elements are denoted by $x_{m,j} \in \calX=\{a_1, a_2,\cdots, a_Q\}$:
\beq  \calC =\left[\begin{array}{c} \bfx_1 \\ \vdots \\ \bfx_M \end{array} \right]= \left[ \begin{array}{cccc} x_{1,1} & x_{1,2} & \cdots & x_{1,n} \\ \vdots & \vdots & \ddots & \vdots \\ x_{M,1} & x_{M,2} & \cdots & x_{M,n}  \end{array} \right] \eeq Let $P_\err(\bfx_m(\calC))$ denote the block decoding error probability when the $m$-th codeword $\bfx_m$ of a particular code $\calC$ is transmitted. Let  $P_\err(\calC)$ denote the block error probability of a particular code $\calC$. Let $\Pr(m)$ denote the probability that the $m$-th message is transmitted or the $m$-th codeword is chosen to be transmitted. Then we have \beq P_\err(\calC) =  \sum_{m=1}^M \Pr(m) P_\err(\bfx_m(\calC)) \eeq As a special case, when a priori message probabilities are equal ($\Pr(m)=\frac{1}{M}$), we have \beq P_\err(\calC) = \frac{1}{M} \sum_{m=1}^M P_\err(\bfx_m(\calC)) \eeq


\section{Achievability: Error Upper-Bound when $R< C$ \cite[pp. 128--133]{viterbi}}

Assume that codewords $\bfx_m \in \calX^n, m=1,\cdots,M$ are randomly generated by the same distribution $q(\bfx)$ to create an ensemble of many random codes. Assume the $m$-th codeword is transmitted for each of the random codes in the ensemble. Then the average error probability for the $m$-th codeword over the ensemble of {\it all} possible random codes is given by \cite[eq. (3.1.2)]{viterbi} \beq \bar P_\err(m) = \sum_{\calC} \Pr(\calC) P_\err(\bfx_m(\calC)), ~~~ m=1,\cdots,M \eeq where \beq \Pr(\calC) = q(\bfx_1(\calC))q(\bfx_2(\calC))\cdots q(\bfx_M(\calC)) \eeq
After some manipulations, $\bar P_\err(m)$ is upper-bounded by \cite[eq. (3.1.11)]{viterbi} \beq \bar P_\err(m) \leq P_\err^\up(q(\bfx)), ~~~m=1,\cdots, M \eeq where $P_\err^\up(q(\bfx))$ is independent of $m$ and given by \cite[eq. (3.1.11)]{viterbi} \beq P_\err^\up(q(\bfx)) = M^\rho \sum_\bfy \left[ \sum_{\bfx \in \calX^n} q(\bfx) p(\bfy|\bfx)^{1/(1+\rho)}\right]^{1+\rho}, ~~~~ 0 \leq \rho \leq 1 \label{eq:P_err_up_q_bfx} \eeq

For DMCs, we have $p(\bfy|\bfx)=\prod_{j=1}^n p(y_j|x_j)$. Also, we {\it suppose} the distribution $q(\bfx)$ is given in a product form of a single distribution $q(x)$ \cite[eq. (3.1.13)]{viterbi}:\footnote{This means that every element $x_{mj}$ in $\calC$ is randomly generated by a single distribution $q(x)$.} \beq q(\bfx) = \prod_{j=1}^n q(x_j) \eeq Then we have \cite[eq. (3.1.14)]{viterbi} \beq \bar P_\err(m) \leq P_\err^\up(q(\bfx)) = P_\err^\up(q(x)) \eeq where $P_\err^\up(q(x))$ is is independent of $m$ and given by \cite[eq. (3.1.14)]{viterbi} \beq P_\err^\up(q(x))= M^\rho \left\{ \sum_y \left[ \sum_{x \in \calX} q(x) p(y|x)^{1/(1+\rho)}\right]^{1+\rho} \right\}^n, ~~~ 0 \leq \rho \leq 1 \label{eq:P_err_u_any_q_x} \eeq

Finally, the  average error probability over the ensemble of all random codes of which elements are randomly generated by $q(x)$ is given by \beqa \bar P_\err &=& \sum_{m=1}^M \Pr(m) \bar P_\err(m) \\ &\stackrel{(a)}{=}& \bar P_\err(m) \\ & \leq & P_\err^\up(q(x)) \eeqa where $(a)$ is valid for arbitrarily a priori message probabilities, not necessarily $\Pr(m)=\frac{1}{M}$. Because $P_\err^\up(q(x))$ is an upper-bound of ensemble average of error probabilities of all possible $\calC$ and $P_\err^\up(q(x))$ is independent of $\calC$, we can conclude that

``{\it At least one code} in the ensemble generated by $q(x)$ must have the error probability no greater than the ensemble average bound, i.e., \beq P_\err(\calC) \leq P_\err^\up(q(x)),~~~ \exists \calC {\rm ~in~the ~ensemble~generated~by~} q(x)  \eeq where it can be shown that \cite[p. 136]{viterbi} \beq \lim_{n\rightarrow \infty} P_\err^\up(q(x)) = 0,~~ R< I(q(x))"\eeq \hfill $\Box$

We can further tighten the bound by considering an optimal $q(x)$ to generate the ensemble as follows: \beq \bar P_\err \leq \min_{q(x)} P_\err^\up(q(x)) \eeq
Overall, achievability means \cite[p. 133]{viterbi}:

``{\it At least one code} in the ensemble generated by optimal $q(x)$ must have the error probability no greater than the tightest ensemble average bound, i.e., \beq P_\err(\calC) \leq \min_{q(x)} P_\err^\up(q(x)),~~~ \exists \calC {\rm ~in~the ~ensemble~generated~by~optimal~} q(x) \eeq where it can be shown that \cite[p. 137]{viterbi} \beq \lim_{n\rightarrow  \infty} \min_{q(x)} P_\err^\up(q(x)) = 0,~~ R< C=\max_{q(x)}I(q(x)) "\eeq \hfill $\Box$

{\it Remark 1:} It is possible derive a bit stronger result \cite[Corollary, p. 138]{viterbi}: \beq P_\err(\bfx_m(\calC)) \leq \min_{q(x)} 4 P_\err^\up(q(x)),~~~\forall m; ~~ \exists \calC {\rm ~in~the ~ensemble~generated~by~optimal~} q(x); ~~ R<C. \eeq \hfill $\Box$




\section{Strong Converse: Error Lower-Bound when $R> C$ \\ \cite{Arimoto}, \cite[pp. 186--189]{viterbi}, \cite[pp. 202--204]{Blahut}} We consider a specific code \beq \calC=\left[ \begin{array}{c} \bfx_1(\calC) \\ \vdots \\ \bfx_M(\calC) \end{array} \right] \eeq Note that $\calC$ can be any deterministic code or a realization of any random code in any possible ensemble generated by any possible input distribution. If we assume that a priori message probabilities are equal (i.e., $\Pr(m)=\frac{1}{M}$)\footnote{This assumption is also used in Wolfowitz's strong converse for $R>C$ \cite[p. 174]{gallager}, and in Sphere Packing lower-bound for $R<C$ \cite[p. 157]{gallager}. However, such assumption is not needed for weak converse based on Fano's inequality \cite[p. 207]{cover}.}, the error probability for the specific code $\calC$ is given by \cite[eq. (3.9.9)]{viterbi}: \beqa P_\err(\calC) & = & 1- \sum_{m=1}^M \Pr(m) \sum_{\bfy \in \Lambda_m} p(\bfy|\bfx_m(\calC)) \\ &=&  1-\frac{1}{M} \sum_{m=1}^M \sum_{\bfy \in \Lambda_m} p(\bfy|\bfx_m(\calC)) \eeqa where $\Lambda_m$ is the optimum decision region for $\bfx_m$: $\Lambda_m =\{\bfy: \max_{m'} p(\bfy|\bfx_{m'}(\calC)) = p(\bfy|\bfx_m(\calC))\}$.
It also can be lower-bounded as follows \cite[eq. (3.9.11)]{viterbi} \beqa P_\err(\calC) & \geq & P_\err^\low(\calC)  \eeqa where $P_\err^\low(\calC)$ is given by \cite[eq. (3.9.11)]{viterbi}: \beq P_\err^L(\calC) = 1 - \frac{1}{M}\sum_\bfy \left(\sum_{m=1}^M p(\bfy|\bfx_m(\calC))^{1/\beta}\right)^\beta \eeq


We now represent the specific codeword $\calC$ in terms of {\it special} probability distribution $q_\calC(\bfx)$, which is given by \cite[eq. (3.9.12)]{viterbi} \beq q_\calC(\bfx) = \left\{ \begin{array}{ll} \frac{1}{M}, & \bfx = \bfx_m(\calC), ~~~ m=1,\cdots, M \\ 0, & {\rm otherwise~} (\bfx \in \calX^n, \bfx \neq \bfx_m(\calC)) \end{array} \right. \label{eq:q_bfx_code_prob} \eeq or $q_\calC(\bfx)$ can be written as \cite[Proof of Themreom 6.1.1]{Blahut} \beq q_\calC(\bfx) = \left\{ \begin{array}{ll} \frac{1}{M}, & {\rm if ~} \bfx {\rm ~ is ~ one~ of~the ~ codewords ~ of ~the ~ current ~specific ~ code ~ } \calC \\ 0, & {\rm otherwise~} (\bfx \in \calX^n, \bfx \neq \bfx_m(\calC)) \end{array} \right. \eeq where we used the condition of $\Pr(m)=\frac{1}{M}$.
Note that the current specific code $\calC$ is uniquely determined by $q_\calC(\bfx)$; and $q_\calC(\bfx)$ is uniquely determined by the current code $\calC$, not by the input distribution (see the example in the next subsection). In fact, when $\calC$ is a deterministic code, the input distribution does not need to be even defined at all.
Using $q_\calC(\bfx)$, we rewrite the lower-bound of the specific code $\calC$ as follows: \beqa P_\err(\calC) & \geq & P_\err^\low(\calC) = P_\err^\low(q_\calC(\bfx)) \eeqa where $P_\err^\low(q_\calC(\bfx))$ is given by \cite[eq. (3.9.13)]{viterbi}: \beqa P_\err^L(q_\calC(\bfx)) &=& 1 -\frac{1}{M} \sum_\bfy \left(M\sum_{\bfx \in \calX^n} q_\calC(\bfx) p(\bfy|\bfx)^{1/\beta}\right)^\beta \\ &=& 1 -M^{\rho'} \sum_\bfy \left(\sum_{\bfx \in \calX^n} q_\calC(\bfx) p(\bfy|\bfx)^{1/(1+\rho')}\right)^{1+\rho'}, ~~~ -1 < \rho' \leq 0 \label{eq:P_err^L_q_bfx_init} \eeqa where $\beta = 1 + \rho'$. Note that this expression is not in a single letter form (of which computational complexity is independent of blocklength $n$). For large $n$, (\ref{eq:P_err^L_q_bfx_init}) is an intractable expression, of which computation is infeasible.


Unfortunately, it is generally {\it not} possible to further simply the lower-bound expression $P_\err^L(q_\calC(\bfx))$ of (\ref{eq:P_err^L_q_bfx_init}) into a single-letter form. The reason is as follows. For a specific code $\calC$ or for the specific $q_\calC(\bfx)$ uniquely determined by a specific code $\calC$, it is generally {\it not} possible to write $q_\calC(\bfx)$ of (\ref{eq:q_bfx_code_prob}) as $q_\calC(\bfx)= \prod_{j=1}^n q_\calC(x_j)$,  although we can still write $p(\bfy|\bfx)$ as $p(\bfy|\bfx) = \prod_{j=1}^n p(y_j|x_j)$ for DMCs. Furthermore, $P_\err^L(q_\calC(\bfx))$ in (\ref{eq:P_err^L_q_bfx_init}) is a valid lower-bound {\it only} for the current specific code $\calC$, not necessarily valid for other codes.


The above two issues can be addressed, if we further lower-bound $P_\err^L(q_\calC(\bfx))$ in (\ref{eq:P_err^L_q_bfx_init}) as follows: \beqa P_\err(\calC) &\geq & P_\err^\low(q_\calC(\bfx)) \\ & \geq & \min_{q(\bfx)} P_\err^\low(q(\bfx)) \eeqa where $\min_{q(\bfx)} P_\err^\low(q(\bfx))$ is given by \cite[eq. (3.9.14)]{viterbi} \beq \min_{q(\bfx)} P_\err^\low(q(\bfx)) = 1-M^{\rho'} \max_{q(\bfx)} \sum_\bfy \left( \sum_{\bfx \in \calX^n} q(\bfx) p(\bfy|\bfx)^{1/(1+\rho')}\right)^{1+\rho'}, ~~~ -1< \rho' \leq 0 \eeq

Now, from the Kuhn-Tucker theorem, we can derive the necessary and sufficient condition that $q(\bfx)$ must satisfy in order to minimize $P_\err^L(q(\bfx))$, and the condition is given by \cite[eq. (3.9.18)]{viterbi}. It is easy to see that the condition \cite[eq. (3.9.18)]{viterbi} can be still satisfied even if we write $q(\bfx)$ in the product form \cite[eq. (3.9.19)]{viterbi}, \cite[Lemma 2]{Arimoto} \beq q(\bfx)=\prod_{j=1}^n q(x_j) \eeq For DMCs, therefore, we can rewrite the lower-bound as
\beqa P_\err(\calC)  & \geq & \min_{q(\bfx)} P_\err^\low(q(\bfx)) \\ &=& \min_{q(x)} P_\err^\low(q(x)) \eeqa
where $\min_{q(x)} P_\err^\low(q(x))$ is given by \cite[eq. (3.9.21)]{viterbi} \beq \min_{q(x)} P_\err^\low(q(x)) =1 - M^{\rho'} \max_{q(x)} \left[ \sum_y \left( \sum_{x \in \calX} q(x) p(y|x)^{1/(1+\rho')} \right)^{1+\rho'} \right]^n, ~~~ -1< \rho' \leq 0 \label{eq:P_err_L_q_x_final} \eeq Note that the lower-bound of $\min_{q(x)} P_\err^\low(q(x))$ in (\ref{eq:P_err_L_q_x_final}) is given in a single-letter form. Finally, note the derivation above is valid for {\it any code} $\calC$.

%\newpage

Overall, the strong converse means \cite[Theorem 3.9.1]{viterbi}:

`` The error probability of {\it  any code} is lower-bounded by $\min_{q(x)} P_\err^\low(q(x))$, i.e.,  \beq P_\err(\calC) \geq \min_{q(x)} P_\err^\low(q(x)), ~~~ \forall \calC \eeq where it can be shown that \beq \lim_{n \rightarrow \infty} \min_{q(x)} P_\err^\low(q(x))=1, ~~~ R>C." \eeq

{\it Remark 2:} The above result is valid only when each codeword within a code is used (or chosen) with equal probability to send data, i.e., {\it a priori message probabilities are equal.} This does {\it not} mean that the code must be randomly generated by an equi-probable distribution. The code can be any deterministic code or any random code generated by any non-equi-probable distributions. However, once a code is constructed, the rows must be chosen with equal probability.


{\it Remark 3:} In the above result \cite[Theorem 3.9.1]{viterbi}, ``any code" means truly all codes of length $n$ with $R>C$, not necessarily all codes in the same ensemble generated by a particular input distribution. That is, ``any code" means all possible deterministic codes or realizations of all random codes in all possible ensembles generated by all possible input distributions.


%\newpage
\section{Notation Issue of $q(\bfx)$}

In \cite{viterbi}, the same notation $q(\bfx)$ is used for achievability \cite[pp. 123--133]{viterbi} and the strong converse \cite[pp. 186--189]{viterbi}. Although the notation is mathematically correct, such usage of the notation is confusing and somewhat misleading, because the meanings are different. As an example, in \cite{viterbi}, for the two expressions of (\ref{eq:P_err_up_q_bfx}) and (\ref{eq:P_err^L_q_bfx_init}), the same notation $q(\bfx)$ is used; and thus, (\ref{eq:P_err_up_q_bfx}) and (\ref{eq:P_err^L_q_bfx_init}) might appear to be equivalent. However, the two forms are {\it not} equivalent because $q(\bfx)$ are defined differently.

To address the issue, in our document, we use different notation: $q(\bfx)$ for  (\ref{eq:P_err_up_q_bfx}) and $q_\calC(\bfx)$ for (\ref{eq:P_err^L_q_bfx_init}). Recall that in (\ref{eq:P_err_up_q_bfx}), $q(\bfx)$ represents the probability distribution that randomly generates codewords of random codes in an ensemble. In (\ref{eq:P_err^L_q_bfx_init}), $q_\calC(\bfx)$ represents the special probability distribution that uniquely specifies a particular code $\calC$. 

Both $q(\bfx)$ and $q_\calC(\bfx)$ can be considered as {\it two functions} taking inputs from the same set and giving outputs as probabilities: both takes an input as a vector in the set $\calX^n$; and their outputs are probabilities: \beq q(\bfx = \bfx_0) = {\rm probability}_1 {\rm ~~~ and ~~~} q_\calC(\bfx = \bfx_0) = {\rm probability}_2, ~~ \bfx_0 \in \calX^n \eeq However, the two functions are different, and thus, the values of the outputs are generally different: \beq {\rm probability}_1 \neq {\rm probability}_2 \eeq

In order to clarify this difference between $q(\bfx)$ and $q_{\calC}(\bfx)$, we consider an example.

\newpage

{\it [Example]:} Let us consider the case $Q=2$, $n=3$, and $M=2$, where $\calX=\{a_1,a_2\}$. Then $\calX^n$ is given by \begin{small} \beqa \calX^n=\{ (a_1,a_1,a_1), (a_1,a_1,a_2), (a_1,a_2,a_1), (a_1,a_2,a_2), (a_2,a_1,a_1), (a_2,a_1,a_2), (a_2, a_2, a_1), (a_2, a_2, a_2) \} \non \eeqa \end{small} Let $\calC$ denote the code given by \beqa \calC &=& \left[ \begin{array}{c} \bfx_1 \\ \bfx_2 \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1} & x_{1,2} & x_{1,3} \\ x_{2,1} & x_{2,2} & x_{2,3} \end{array} \right]  \eeqa

\subsection{Achievability: Error Upper-Bound when $R< C$}

In order to generate an ensemble of random codes, we suppose that each codeword $\bfx_m$ is drawn from $\calX^n$ by probability distribution $q(\bfx)$ given by
\beq q(\bfx) = q(\bfx_m)= \left\{ \begin{array}{ll} \frac{1}{27}, & {\rm if~} \bfx_m = (a_1,a_1,a_1) \\ \frac{2}{27}, & {\rm if~} \bfx_m \in \{ (a_1,a_1,a_2), (a_1, a_2, a_1), (a_2, a_1, a_1) \} \\ \frac{4}{27}, & {\rm if~} \bfx_m \in \{ (a_1,a_2,a_2), (a_2, a_1, a_2), (a_2, a_2, a_1) \} \\ \frac{8}{27}, & {\rm if~} \bfx_m = (a_2,a_2,a_2) \end{array} \right., ~~~ m=1,2 \label{eq:q_x_m_achievability} \eeq where \beqa \sum_{\bfx_1 \in \calX^n} q(\bfx_1) &= & 1 \\  \sum_{\bfx_2 \in \calX^n} q(\bfx_2) &= & 1  \eeqa
Or, in general, \beq \sum_{\bfx_m \in \calX^n} q(\bfx_m) =1, ~~~{\rm for ~ all~} m=1,2,\cdots,M \eeq

For example, the ensemble of random codes can be generated as follows: \beqa \calC^{(1)} &=& \left[ \begin{array}{c} \bfx_1^{(1)} \\ \bfx_2^{(1)} \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1}^{(1)} & x_{1,2}^{(1)} & x_{1,3}^{(1)}  \\ x_{2,1}^{(1)} & x_{2,2}^{(1)} & x_{2,3}^{(1)} \end{array} \right] = \left[ \begin{array}{ccc} a_1 & a_1 & a_1 \\ a_1 & a_1 & a_1 \end{array} \right] \\ \calC^{(2)} &=& \left[ \begin{array}{c} \bfx_1^{(2)} \\ \bfx_2^{(2)} \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1}^{(2)} & x_{1,2}^{(2)} & x_{1,3}^{(2)}  \\ x_{2,1}^{(2)} & x_{2,2}^{(2)} & x_{2,3}^{(2)} \end{array} \right] = \left[ \begin{array}{ccc} a_1 & a_1 & a_1 \\ a_1 & a_1 & a_2 \end{array} \right] \\ \calC^{(3)} &=& \left[ \begin{array}{c} \bfx_1^{(3)} \\ \bfx_2^{(3)} \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1}^{(3)} & x_{1,2}^{(3)} & x_{1,3}^{(3)}  \\ x_{2,1}^{(3)} & x_{2,2}^{(3)} & x_{2,3}^{(3)} \end{array} \right] = \left[ \begin{array}{ccc} a_1 & a_1 & a_1 \\ a_1 & a_2 & a_1 \end{array} \right] \\ \vdots & & ~~~~~ \vdots \\ \calC^{(64)} &=& \left[ \begin{array}{c} \bfx_1^{(64)} \\ \bfx_2^{(64)} \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1}^{(64)} & x_{1,2}^{(64)} & x_{1,3}^{(64)}  \\ x_{2,1}^{(64)} & x_{2,2}^{(64)} & x_{2,3}^{(64)} \end{array} \right] = \left[ \begin{array}{ccc} a_1 & a_1 & a_1 \\ a_1 & a_2 & a_1 \end{array} \right] \eeqa where $\calC^{(1)}$, $\calC^{(2)}$, $\calC^{(3)}$, $\cdots$, $\calC^{(64)}$ are generated with probability $\frac{1}{27^2}$, $\frac{2}{27^2}$, $\frac{2}{27^2}$, $\cdots$, $\frac{64}{27^2}$, respectively.

When $q(\bfx)$ is given by (\ref{eq:q_x_m_achievability}), it can be written in a product form of $q(x)$ as follows: \beq q(\bfx_m) = q(x_{m,1})q(x_{m,2})q(x_{m,3}), ~~~ m=1,2 \eeq or simply, \beq q(\bfx) = q(x_{1})q(x_{2})q(x_{3}) \eeq
where the input distribution $q(x)$ is given by
\beq q(x) = \left\{ \begin{array}{ll} \frac{1}{3}, & {\rm if~} x = a_1 \\ \frac{2}{3}, & {\rm if~} x = a_2 \end{array} \right. \label{eq:input_dist} \eeq
That is, the ensemble can be created by randomly and independently generating each element of $\calC^{(i)}$ using $q(x)$.

{\it Remark 4:} The upper-bound of error probability averaged over the ensemble of all codes $\{ \calC^{(i)}:i=1,\cdots,64\}$ in the example can be obtained by $P_\err^\up(q(x))$ of (\ref{eq:P_err_u_any_q_x}) along with $q(x)$ of (\ref{eq:input_dist}). However, in order to show the existence of the {\it best} code(s) (in terms of smallest error probability or largest rate), one must consider the ensemble of random codes with optimal occurrence probability distribution.
For symmetric DMCs, the optimal distribution minimizing the upper-bound of error probability is the equi-probable distribution $q_{\rm equ}(x)=\frac{1}{2}$ if $x=a_1$ or $x=a_2$ \cite[Theorem 7.2]{jelinek}. For the best code(s), we need to generate the ensemble of codes using $q_{\rm equ}(x)$. Then the error upper-bound averaged for the ensemble is given by $P_\err^\up(q_{\rm equ}(x))$. From this, the channel capacity $C$ can be determined: $C$ is the maximum rate $R$ subject to $P_\err^\up(q_{\rm equ}(x))\rightarrow 0 $ as $n \rightarrow \infty$. Finally, note that both $q(x)$ of (\ref{eq:input_dist}) and $q_{\rm equ}(x)$ will generated the same ensemble of codes $\{ \calC^{(i)}:i=1,\cdots,64\}$; however, the occurrence probability distributions are different.

\subsection{Strong Converse: Error Lower-Bound when $R > C$}

In the proof of strong converse, we first consider a specific code. For example, let us consider $\check \calC$: \beqa \check \calC &=& \left[ \begin{array}{c}  \bfx_1(\check \calC) \\ \bfx_2(\check \calC) \end{array} \right] =  \left[ \begin{array}{ccc}  x_{1,1}(\check \calC) &  x_{1,2}(\check \calC) &  x_{1,3}(\check \calC)  \\  x_{2,1}(\check \calC) &  x_{2,2}(\check \calC) &  x_{2,3}(\check \calC) \end{array} \right] = \left[ \begin{array}{ccc} a_1 & a_1 & a_2 \\ a_1 & a_2 & a_2 \end{array} \right] \eeqa
Note that this specific code $\check \calC$ might be one realization of random codes generated by $q(\bfx)$ of (\ref{eq:q_x_m_achievability}), or by $q(x)$ of (\ref{eq:input_dist}), or any other input distribution. Or, for the purpose of strong converse, $\check \calC$ might be simply a deterministic code without defining any input distribution such as (\ref{eq:q_x_m_achievability}) and (\ref{eq:input_dist}) at all.


For this specific code $\check \calC$, under the condition that a priori message probabilities are equal, the special distribution $q_{\check \calC}(\bfx)$ of (\ref{eq:q_bfx_code_prob}) is given by
\beqa q_{\check \calC}(\bfx= \bfx_1(\check \calC)) &=& q_{\check \calC}(\bfx=(a_1,a_1,a_2)) = \frac{1}{2} \\ q_{\check \calC}(\bfx= \bfx_2(\check \calC)) &=& q_{\check \calC}(\bfx=(a_1,a_2,a_2)) = \frac{1}{2} \eeqa
or
\beqa q_{\check \calC}(\bfx) = \left\{ \begin{array}{ll} \frac{1}{2}, & {\rm if~} \bfx = \bfx_1(\check \calC)= (a_1, a_1, a_2) {\rm ~ or~} \bfx=\bfx_2(\check \calC) = (a_1, a_2, a_2) \\ 0, & {\rm otherwise} \end{array} \right. \label{eq:strong_converse_q_bfx} \eeqa
Note that this $q_{\check \calC}(\bfx)$ in (\ref{eq:strong_converse_q_bfx}) is purely determined by the code $\check \calC$, not by the input distribution $q(x)$ in (\ref{eq:input_dist}). Specifically,  a code $\check \calC$ is one-to-one mapped to the distribution $q_{\check \calC}(\bfx)$ in (\ref{eq:strong_converse_q_bfx}): If $q_{\check \calC}(\bfx)$ of (\ref{eq:strong_converse_q_bfx}) is given, the corresponding code is uniquely determined; or, if a code is given, the corresponding distribution $q_{\check \calC}(\bfx)$ in (\ref{eq:strong_converse_q_bfx}) is uniquely determined. Note that it is generally {\it not} possible to write $q_{\check \calC}(\bfx)$ of (\ref{eq:strong_converse_q_bfx}) in the form of $q_{\check \calC}(\bfx)=q_{\check \calC}(x_1)q_{\check \calC}(x_2)q_{\check \calC}(x_3)$.

In general, over all $M$ codewords $\{ \bfx_m (\calC):m=1,\cdots,M\}$ of any arbitary code $\calC$, we have \beqa \sum_{m=1}^M q_\calC(\bfx_m(\calC)) &=& 1, ~~~~ \forall \calC \eeqa


{\it Remark 5:} The lower-bound of error probability for the specific code $\check \calC$ can be obtained by substituting $q_{\check \calC}(\bfx)$ of (\ref{eq:strong_converse_q_bfx}) into the error expression of (\ref{eq:P_err^L_q_bfx_init}). However, the obtained expression is not in a single letter form. For large $n$, it is an intractable expression, of which computation is infeasible. For $\check \calC$, a tractable expression of lower-bound of error probability is obtained by using the worst distribution as in (\ref{eq:P_err_L_q_x_final}). For symmetric DMCs, it can be shown that the worst distribution is equi-probable distribution $q_{\rm qui}(x)$ (see Appendix A of the report).


Overall, for code $\check \calC$, three different types of probability distributions are involved:
\bitem
\item $q(\bfx)$ of (\ref{eq:q_x_m_achievability}) or $q(x)$ of (\ref{eq:input_dist}): $\check \calC$ might be a realization of the code generated by $q(\bfx)$ of (\ref{eq:q_x_m_achievability}) or $q(x)$ of (\ref{eq:input_dist}) or any other distribution. Or, $\check \calC$ might be a deterministic code without requiring any input distribution.
\item $q_{\check \calC}(\bfx)$ of (\ref{eq:strong_converse_q_bfx}): The code $\check \calC$ is uniquely mapped to $q_{\check \calC}(\bfx)$ of (\ref{eq:strong_converse_q_bfx}), which can be used for (\ref{eq:P_err^L_q_bfx_init}).
\item $q_{\rm equ}(x)$: For the code $\check \calC$, over symmetric DMCs, the single-letter expression of error probability lower-bound is given by $q_{\rm equ}(x)$, which is used for (\ref{eq:P_err_L_q_x_final}).
\eitem
Note that the special distribution $q_{\check \calC}(\bfx)$ of (\ref{eq:strong_converse_q_bfx}) used to specify a code $\check \calC$ can be generally different from the worst distribution (e.g., $q_{\rm equ}(x)$) used to obtain a (universal) single-letter lower-bound of error probability of the code $\check \calC$.



%\newpage
\section{Some Discussions}

\bitem

\item {\it Single-letter expression of lower-bound when $R>C$:} As discussed before, for a specific code $\calC$, it is generally not possible to write its lower-bound in a single-letter form. Only when we consider the weakest (most loose) lower-bound, it is given in a single-letter form. Also, this weakest lower-bound is valid for all codes as long as $R> C$.

\item {\it Existence of code for Alice:} Consider the system where Alice transmits data at rate $R$ to Bob in the presence of Eve. Assume $R<C_\bob$ and $R>C_\eve$. For a specific code $\check \calC$, we can write the error lower-bound $P_\err^\low(q_{\check \calC}(\bfx))$ of (\ref{eq:P_err^L_q_bfx_init}) at Eve anyway (although the expression is not in a single-letter form). For $\check \calC$, however, there is no guarantee that the error upper-bound $P_\err^\up(q(x))$ at Bob is valid, because $P_\err^\up(q(x))$ is obtained by averaging over the ensemble and thus valid only for some codes in the ensemble; but, there is no guarantee that $\check \calC$ is such codes.

    On the other hand, the weakest lower-bound $\min_{q(x)} P_\err^\low(q(x))$ is valid for any code in the ensemble. Then it is guaranteed that the error upper-bound $P_\err^\up(q(x))$ at Bob is valid.

\item {\it Determination of Input Distribution at Alice:}
    Let $\breve q(x)$ denote the distribution giving the tightest upper-bound: \beq \breve q(x) = \arg \min_{q(x)} P_\err^\up(q(x)), ~~~~ R<C_\bob \eeq Let $\breve q'(x)$ denote the distribution giving the weakest lower-bound \beq \breve q'(x) = \arg \min_{q'(x)} P_\err^\low(q'(x)), ~~~~ R>C_\eve \eeq
    In order to use the tightest upper-bound we should generate the ensemble using $\breve q(x)$. Note that the weakest lower-bound is still obtained by $\breve q'(x)$.

\eitem






\newpage
\vspace{1cm}
\bibliographystyle{IEEE}
\begin{thebibliography}{999}

\bibitem{gallager} R. G. Gallager, {\it Information Theory and Reliable Communications.} New York: Wiley, 1968.

\bibitem{Arimoto} S. Arimoto, ``On the converse to the coding theorem for discrete memoryless channels," {\it IEEE Trans. Inf. Theory,} vol. , pp. 357--359, May 1973.

\bibitem{viterbi} A. J. Viterbi and J. K. Omura, {\it Principles of Digital Communication and Coding.}  New York: McGraw-Hill, 1979.

\bibitem{Blahut} R. E. Blahut, {\it Principles and Practice of Information Theory.} Addison-Wesley, 1987.

\bibitem{jelinek} F. Jelinek, {\it Probabilistic Information Theory.} New York: McGraw-Hill, 1968.

\bibitem{cover} T. M. Cover and J. A. Thomas, {\it Elements of Information Theory.} Wiely, 2nd Ed., 2006.

\end{thebibliography}










































































%%%%%

==> comparison_achievability_converse_new.tex <==
\clearpage
\newpage

\begin{center}
{\bf \Large Comparisons of Proofs of Achievability and Strong Converse}

\vspace{0.5cm}
Il-Min Kim

April 25, 2014

\vspace{1cm}
\end{center}

Consider a code composed of $M=e^{nR}$ signal vectors (or codewords) $\bfx_m, m=1,\cdots,M$ of length $n$, whose elements are denoted by $x_{m,j} \in \calX$, where $\calX = A_Q  = \{a_1, a_2,\cdots, a_Q\}$ or $\calX = \mathbb{R}$:
\beq  \calC =\left[\begin{array}{c} \bfx_1 \\ \vdots \\ \bfx_M \end{array} \right]= \left[ \begin{array}{cccc} x_{1,1} & x_{1,2} & \cdots & x_{1,n} \\ \vdots & \vdots & \ddots & \vdots \\ x_{M,1} & x_{M,2} & \cdots & x_{M,n}  \end{array} \right] \eeq Let $P_\err(\bfx_m(\calC))$ denote the block decoding error probability when the $m$-th codeword $\bfx_m$ of a particular code $\calC$ is transmitted. Let  $P_\err(\calC)$ denote the block error probability of a particular code $\calC$. Let $\Pr(m)$ denote the probability that the $m$-th message is transmitted or the $m$-th codeword is chosen to be transmitted. Then we have \beq P_\err(\calC) =  \sum_{m=1}^M \Pr(m) P_\err(\bfx_m(\calC)) \eeq As a special case, when a priori message probabilities are equal ($\Pr(m)=\frac{1}{M}$), we have \beq P_\err(\calC) = \frac{1}{M} \sum_{m=1}^M P_\err(\bfx_m(\calC)) \eeq


\section{Achievability: Error Upper-Bound when $R< C$ \cite[pp. 128--133]{viterbi}}

Assume that codewords $\bfx_m \in \calX^n, m=1,\cdots,M$ are randomly generated by the same distribution $q(\bfx)$ to create an ensemble of many random codes. Assume the $m$-th codeword is transmitted for each of the random codes in the ensemble. Then the average error probability for the $m$-th codeword over the ensemble of {\it all} possible random codes is given by \cite[eq. (3.1.2)]{viterbi} \beq \bar P_\err(m) = \sum_{\calC \in \calA_\calC(q(\bfx))} \Pr(\calC) P_\err(\bfx_m(\calC)), ~~~ m=1,\cdots,M; ~~~ \bfx_m(\calC)\in A_Q^n \eeq or
\beq \bar P_\err(m) = \int_{\calC \in \calA_\calC(q(\bfx))}  P_\err(\bfx_m(\calC)) d\Pr(\calC), ~~~ m=1,\cdots,M ; ~~~ \bfx_m(\calC) \in \mathbb{R}^n \eeq
where $\calA_\calC(q(\bfx))$ denotes the ensemble of random codes generated by $q(\bfx)$ and \beq \Pr(\calC) = q(\bfx_1(\calC))q(\bfx_2(\calC))\cdots q(\bfx_M(\calC)) \eeq
After some manipulations, $\bar P_\err(m)$ is upper-bounded by \cite[eq. (3.1.11)]{viterbi} \beq \bar P_\err(m) \leq P_\err^\up(q(\bfx)), ~~~m=1,\cdots, M \eeq where $P_\err^\up(q(\bfx))$ is independent of $m$ and given by \cite[eq. (3.1.11)]{viterbi} \beq P_\err^\up(q(\bfx)) = M^\rho \sum_\bfy \left[ \sum_{\bfx \in \calX^n} q(\bfx) p(\bfy|\bfx)^{1/(1+\rho)}\right]^{1+\rho}, ~~~~ 0 \leq \rho \leq 1; ~~~ \calX^n = A_Q^n \label{eq:P_err_up_q_bfx} \eeq or \beq P_\err^\up(q(\bfx)) = M^\rho \int_\bfy \left[ \int_{\bfx \in \calX^n} q(\bfx) p(\bfy|\bfx)^{1/(1+\rho)} d\bfx \right]^{1+\rho} d\bfy, ~~~~ 0 \leq \rho \leq 1; ~~~ \calX^n = \mathbb{R}^n \eeq

For DMCs, we have $p(\bfy|\bfx)=\prod_{j=1}^n p(y_j|x_j)$. Also, we {\it suppose} the distribution $q(\bfx)$ is given in a product form of a single distribution $q(x)$ \cite[eq. (3.1.13)]{viterbi}:\footnote{This means that every element $x_{mj}$ in $\calC$ is randomly generated by a single distribution $q(x)$.} \beq q(\bfx) = \prod_{j=1}^n q(x_j) \eeq Then we have \cite[eq. (3.1.14)]{viterbi} \beq \bar P_\err(m) \leq P_\err^\up(q(\bfx)) = P_\err^\up(q(x)) \eeq where $P_\err^\up(q(x))$ is is independent of $m$ and given by \cite[eq. (3.1.14)]{viterbi} \beq P_\err^\up(q(x))= M^\rho \left\{ \sum_y \left[ \sum_{x \in \calX} q(x) p(y|x)^{1/(1+\rho)}\right]^{1+\rho} \right\}^n, ~~~ 0 \leq \rho \leq 1 \label{eq:P_err_u_any_q_x} ; ~~~ \calX = A_Q \eeq or \beq P_\err^\up(q(x))= M^\rho \left\{ \int_y \left[ \int_{x \in \calX} q(x) p(y|x)^{1/(1+\rho)} dx \right]^{1+\rho} dy \right\}^n, ~~~ 0 \leq \rho \leq 1 ; ~~~ \calX = \mathbb{R} \eeq

Finally, the  average error probability over the ensemble of all random codes of which elements are randomly generated by $q(x)$ is given by \beqa \bar P_\err &=& \sum_{m=1}^M \Pr(m) \bar P_\err(m) \\ &\stackrel{(a)}{=}& \bar P_\err(m) \\ & \leq & P_\err^\up(q(x)) \eeqa where $(a)$ is valid for arbitrarily a priori message probabilities, not necessarily $\Pr(m)=\frac{1}{M}$. Because $P_\err^\up(q(x))$ is an upper-bound of ensemble average of error probabilities of all possible $\calC$ and $P_\err^\up(q(x))$ is independent of $\calC$, we can conclude that

``{\it At least one code} in the ensemble generated by $q(x)$ must have the error probability no greater than the ensemble average bound, i.e., \beq P_\err(\calC) \leq P_\err^\up(q(x)),~~~ \exists \calC \in \calA_\calC(q(x))  \eeq where it can be shown that \cite[p. 136]{viterbi} \beq \lim_{n\rightarrow \infty} P_\err^\up(q(x)) = 0,~~ R< I(q(x))."\eeq \hfill $\Box$

We can further tighten the bound by considering an optimal $q(x)$ to generate the ensemble as follows: \beq \bar P_\err \leq \min_{q(x)} P_\err^\up(q(x)) = P_\err^\up(\breve q(x)) \eeq where \beq \breve q(x) = \arg \min_{q(x)} P_\err^\up(q(x)) \eeq
Overall, achievability means \cite[p. 133]{viterbi}:

``{\it At least one code} in the ensemble generated by optimal $\breve q(x)$ must have the error probability no greater than the tightest ensemble average bound, i.e., \beq P_\err(\calC) \leq P_\err^\up(\breve q(x)),~~~ \exists \calC \in \calA_{\calC}(\breve q(x)) \eeq where it can be shown that \cite[p. 137]{viterbi} \beq  \lim_{n\rightarrow  \infty} P_\err^\up(\breve q(x)) = 0,~~ R< C=I(\breve q(x)). "\eeq \hfill $\Box$

{\it Remark 1:} It is possible derive a bit stronger result \cite[Corollary, p. 138]{viterbi}: \beq P_\err(\bfx_m(\calC)) \leq 4 P_\err^\up(\breve q(x)),~~~\forall m; ~~ \exists \calC  \in \calA_\calC(\breve q(x)); ~~ R<C. \eeq \hfill $\Box$



\newpage
\section{Strong Converse: Error Lower-Bound when $R> C$ \\ \cite{Arimoto}, \cite[pp. 186--189]{viterbi}, \cite[pp. 202--204]{Blahut}} We consider a specific code \beq \calC=\left[ \begin{array}{c} \bfx_1(\calC) \\ \vdots \\ \bfx_M(\calC) \end{array} \right] \eeq Note that $\calC$ can be any deterministic code or a realization of any random code in any possible ensemble generated by any possible input distribution $q(\bfx)$ or $q(x)$. If we assume that a priori message probabilities are equal (i.e., $\Pr(m)=\frac{1}{M}$)\footnote{This assumption is also used in Wolfowitz's strong converse for $R>C$ \cite[p. 174]{gallager}, and in Sphere Packing lower-bound for $R<C$ \cite[p. 157]{gallager}. However, such assumption is not needed for weak converse based on Fano's inequality \cite[p. 207]{cover}.}, the error probability for the specific code $\calC$ is given by \cite[eq. (3.9.9)]{viterbi}: \beqa P_\err(\calC) & = & 1- \sum_{m=1}^M \Pr(m) \sum_{\bfy \in \Lambda_m} p(\bfy|\bfx_m(\calC)) \\ &=&  1-\frac{1}{M} \sum_{m=1}^M \sum_{\bfy \in \Lambda_m} p(\bfy|\bfx_m(\calC)), ~~~ \bfx_m(\calC) \in A_Q^n \eeqa
or 
\beqa P_\err(\calC) & = & 1- \sum_{m=1}^M \Pr(m) \int_{\bfy \in \Lambda_m} p(\bfy|\bfx_m(\calC)) d \bfy \\ & = &  1-\frac{1}{M} \sum_{m=1}^M \int_{\bfy \in \Lambda_m} p(\bfy|\bfx_m(\calC)) d \bfy, ~~~ \bfx_m(\calC) \in \mathbb{R}^n \eeqa
where $\Lambda_m$ is the optimum decision region for $\bfx_m$: $\Lambda_m =\{\bfy: \max_{m'} p(\bfy|\bfx_{m'}(\calC)) = p(\bfy|\bfx_m(\calC))\}$.


It also can be lower-bounded as follows \cite[eq. (3.9.11)]{viterbi} \beqa P_\err(\calC) & \geq & P_\err^\low(\calC)  \eeqa where $P_\err^\low(\calC)$ is given by \cite[eq. (3.9.11)]{viterbi}: \beq P_\err^L(\calC) = 1 - \frac{1}{M}\sum_\bfy \left(\sum_{m=1}^M p(\bfy|\bfx_m(\calC))^{1/\beta}\right)^\beta, ~~~ \bfx_m(\calC) \in A_Q^n \label{eq:P_err_low_calC} \eeq
or
\beq P_\err^L(\calC) = 1 - \frac{1}{M}\int_\bfy \left(\sum_{m=1}^M p(\bfy|\bfx_m(\calC))^{1/\beta}\right)^\beta d\bfy, ~~~ \bfx_m(\calC) \in \mathbb{R}^n \eeq

{\it Remark 2:} Arimoto's idea is to derive a tractable, universal, and single-letter lower-bound by considering an ensemble as in the case of achievability. Specifically, he mentions \cite[below eq. (6)]{Arimoto}: ``This inequality gives a lower bound for any particular code and maximum-likelihood decoding. However, when $n$ is large, this bound becomes complicated and does not imply any convergence property. It is therefore necessary to simplify inequality (\ref{eq:P_err_low_calC}) by averaging the right-hand side of (\ref{eq:P_err_low_calC}) over the ensemble of all possible codes." \hfill $\Box$


To that end, we now represent the specific codeword $\calC$ in terms of {\it special} probability distribution $q_\calC(\bfx)$, which is given by \cite[eq. (3.9.12)]{viterbi} \beq q_\calC(\bfx) = \left\{ \begin{array}{ll} \frac{1}{M}, & \bfx = \bfx_m(\calC) \in A_Q^n , ~~~ m=1,\cdots, M \\ 0, & {\rm otherwise~} (\bfx \in \calX^n, \bfx \neq \bfx_m(\calC)) \end{array} \right. \label{eq:q_bfx_code_prob} \eeq or $q_\calC(\bfx)$ can be written as \cite[Proof of Themreom 6.1.1]{Blahut} \beq q_\calC(\bfx) = \left\{ \begin{array}{ll} \frac{1}{M}, & {\rm if ~} \bfx {\rm ~ is ~ one~ of~the ~ codewords ~ of ~the ~ current ~specific ~ code ~ } \calC \\ 0, & {\rm otherwise~} (\bfx \in \calX^n, \bfx \neq \bfx_m(\calC)) \end{array} \right. \eeq where we used the condition of $\Pr(m)=\frac{1}{M}$.
Or, for continuous case, $q_\calC(\bfx)$ is given by \beq q_\calC(\bfx) = \frac{1}{M} \delta(\bfx - \bfx_m(\calC)) , ~~~ m=1,\cdots, M; ~~~ \bfx_m(\calC) \in \mathbb{R}^n   \eeq


Note that the current specific code $\calC$ is uniquely determined by $q_\calC(\bfx)$; and $q_\calC(\bfx)$ is uniquely determined by the current code $\calC$, not by the input distribution (see the example in the next subsection). In fact, when $\calC$ is a deterministic code, the input distribution does not need to be even defined at all.
Using $q_\calC(\bfx)$, we rewrite the lower-bound of the specific code $\calC$ as follows: \beqa P_\err(\calC) & \geq & P_\err^\low(\calC) = P_\err^\low(q_\calC(\bfx)) \eeqa where $P_\err^\low(q_\calC(\bfx))$ is given by \cite[eq. (3.9.13)]{viterbi}: \beqa P_\err^L(q_\calC(\bfx)) &=& 1 -\frac{1}{M} \sum_\bfy \left(M\sum_{\bfx \in \calX^n} q_\calC(\bfx) p(\bfy|\bfx)^{1/\beta}\right)^\beta \\ &=& 1 -M^{\rho'} \sum_\bfy \left(\sum_{\bfx \in \calX^n} q_\calC(\bfx) p(\bfy|\bfx)^{1/(1+\rho')}\right)^{1+\rho'}, -1 < \rho' \leq 0;~ \calX^n = A_Q^n \label{eq:P_err^L_q_bfx_init} \eeqa
or
\beqa P_\err^L(q_\calC(\bfx)) &=& 1 -\frac{1}{M} \int_\bfy \left(M\int_{\bfx \in \calX^n} q_\calC(\bfx) p(\bfy|\bfx)^{1/\beta} d \bfx \right)^\beta  d \bfy \\ &=& 1 -M^{\rho'} \int_\bfy \left(\int_{\bfx \in \calX^n} q_\calC(\bfx) p(\bfy|\bfx)^{1/(1+\rho')} d\bfx \right)^{1+\rho'} d\bfy, -1 < \rho' \leq 0; ~ \calX^n = \mathbb{R}^n \non \\ \eeqa
where $\beta = 1 + \rho'$. Note that this expression is not in a single letter form (of which computational complexity is independent of blocklength $n$). For large $n$, (\ref{eq:P_err^L_q_bfx_init}) is an intractable expression, of which computation is infeasible.


Unfortunately, it is generally {\it not} possible to further simply the lower-bound expression $P_\err^L(q_\calC(\bfx))$ of (\ref{eq:P_err^L_q_bfx_init}) into a single-letter form. The reason is as follows. For a specific code $\calC$ or for the specific $q_\calC(\bfx)$ uniquely determined by a specific code $\calC$, it is generally {\it not} possible to write $q_\calC(\bfx)$ of (\ref{eq:q_bfx_code_prob}) as $q_\calC(\bfx)= \prod_{j=1}^n q_\calC(x_j)$,  although we can still write $p(\bfy|\bfx)$ as $p(\bfy|\bfx) = \prod_{j=1}^n p(y_j|x_j)$ for DMCs. Furthermore, $P_\err^L(q_\calC(\bfx))$ in (\ref{eq:P_err^L_q_bfx_init}) is a valid lower-bound {\it only} for the current specific code $\calC$, not necessarily valid for other codes.


The above two issues can be addressed, if we further lower-bound $P_\err^L(q_\calC(\bfx))$ in (\ref{eq:P_err^L_q_bfx_init}) as follows: \beqa P_\err(\calC) &\geq & P_\err^\low(q_\calC(\bfx)) \\ & \geq & \min_{q'(\bfx)} P_\err^\low(q'(\bfx)) \eeqa where $\min_{q'(\bfx)} P_\err^\low(q'(\bfx))$ is given by \cite[eq. (3.9.14)]{viterbi} \beq \min_{q'(\bfx)} P_\err^\low(q'(\bfx)) = 1-M^{\rho'} \max_{q'(\bfx)} \sum_\bfy \left( \sum_{\bfx \in \calX^n} q'(\bfx) p(\bfy|\bfx)^{1/(1+\rho')}\right)^{1+\rho'}, -1< \rho' \leq 0;~ \calX^n = A_Q^n \eeq
or
\beq \min_{q'(\bfx)} P_\err^\low(q'(\bfx)) = 1-M^{\rho'} \max_{q'(\bfx)} \int_\bfy \left( \int_{\bfx \in \calX^n} q'(\bfx) p(\bfy|\bfx)^{1/(1+\rho')} d\bfx \right)^{1+\rho'} d\bfy, -1< \rho' \leq 0;~ \calX^n = \mathbb{R}^n \eeq

Now, from the Kuhn-Tucker theorem, we can derive the necessary and sufficient condition that $q'(\bfx)$ must satisfy in order to minimize $P_\err^L(q'(\bfx))$, and the condition is given by \cite[eq. (3.9.18)]{viterbi}. It is easy to see that the condition \cite[eq. (3.9.18)]{viterbi} can be still satisfied even if we write $q(\bfx)$ in the product form \cite[eq. (3.9.19)]{viterbi}, \cite[Lemma 2]{Arimoto} \beq q'(\bfx)=\prod_{j=1}^n q'(x_j) \eeq For DMCs, therefore, we can rewrite the lower-bound as
\beqa P_\err(\calC)  & \geq & \min_{q'(\bfx)} P_\err^\low(q'(\bfx)) \\ &=& \min_{q'(x)} P_\err^\low(q'(x)) \\ &=&  P_\err^\low(\breve q'(x)) \eeqa
where \beq \breve q'(x) = \arg \min_{q'(x)} P_\err^\low(q'(x)) \eeq
In the above, $\min_{q'(x)} P_\err^\low(q'(x))$ is given by \cite[eq. (3.9.21)]{viterbi} \beqa \min_{q'(x)} P_\err^\low(q'(x))& =& 1 - M^{\rho'} \max_{q'(x)} \left[ \sum_y \left( \sum_{x \in \calX} q'(x) p(y|x)^{1/(1+\rho')} \right)^{1+\rho'} \right]^n\\ &=&1 - M^{\rho'}  \left[ \sum_y \left( \sum_{x \in \calX} \breve q'(x) p(y|x)^{1/(1+\rho')} \right)^{1+\rho'} \right]^n, -1< \rho' \leq 0; ~ \calX = A_Q \label{eq:P_err_L_q_x_final} \non \eeqa  or, \beqa \min_{q'(x)} P_\err^\low(q'(x))& =& 1 - M^{\rho'} \max_{q'(x)} \left[ \int_y \left( \int_{x \in \calX} q'(x) p(y|x)^{1/(1+\rho')} d\bfx \right)^{1+\rho'} d\bfy \right]^n\\ &=&1 - M^{\rho'}  \left[ \int_y \left( \int_{x \in \calX} \breve q'(x) p(y|x)^{1/(1+\rho')} d\bfx \right)^{1+\rho'} d\bfy \right]^n,  -1< \rho' \leq 0; ~ \calX = \mathbb{R} \non \eeqa
Note that the lower-bound of $\min_{q'(x)} P_\err^\low(q'(x))$ in (\ref{eq:P_err_L_q_x_final}) is given in a single-letter form. Finally, note the derivation above is valid for {\it any code} $\calC$.

%\newpage

Overall, the strong converse means \cite[Theorem 3.9.1]{viterbi}:

`` The error probability of {\it  any code} is lower-bounded by $\min_{q(x)} P_\err^\low(q(x))$, i.e.,  \beq P_\err(\calC) \geq P_\err^\low(\breve q'(x)), ~~~ \forall \calC \eeq where it can be shown that \beq \lim_{n \rightarrow \infty}  P_\err^\low(\breve q'(x))=1, ~~~ R>C." \eeq

{\it Remark 3:} The above result is valid only when each codeword within a code is used (or chosen) with equal probability to send data, i.e., {\it a priori message probabilities are equal.} This does {\it not} mean that the code must be randomly generated by an equi-probable distribution. The code can be any deterministic code or any random code generated by any non-equi-probable distributions. However, once a code is constructed, the rows must be chosen with equal probability. \hfill $\Box$


{\it Remark 4:} In the above result \cite[Theorem 3.9.1]{viterbi}, ``any code" means truly all codes of length $n$ with $R>C$, not necessarily all codes in the same ensemble generated by a particular input distribution. That is, ``any code" means all possible deterministic codes or realizations of all random codes in all possible ensembles generated by all possible input distributions. \hfill $\Box$

{\it Remark 5:} Arimoto's approach is essentially the same as in \cite{viterbi}. However, some details (or techniques) are different. Arimoto first considered the worst (or optimal) code $\calC^0$ that minimizes the lower-bound. Then he show that there {\it exists at least one probability distribution} $q'(x)$ that generates an ensemble of random codes whose average is the same as the error lower-bound of the worst code $\calC^0$: \beq P_\err(\calC^0) = \mathbb{E}[P_\err(\calC)] = \sum_{\calC \in \calA_\calC(q'(x))} \Pr(\calC) P_\err(\calC) \eeq where $\calA_\calC(q'(x))$ is the ensemble of random codes generated by $q'(x)$. \hfill $\Box$

%\newpage

{\it Remark 6:} Overall, up to four different types of probability distributions might be involved:
\bitem
\item [i)] $\Pr(m)$: a priori probability distribution or the probability that the $m$-th row of $\calC$ is selected.
    \bitem \item Ex) Equal a priori probabilities: $\Pr(m)=\frac{1}{M}$ \item Ex) Unequal a priori probabilities: $\Pr(m) \neq \frac{1}{M}$ \eitem

\item[ii)] $q(\bfx)$ or $q(x)$: $\calC$ might be a realization of the code generated by $q(\bfx)$ or $q(x)$ or any other distribution. Or, $\calC$ might be a deterministic code without requiring any such input distribution.
    \bitem \item Ex) Equi-probable or non-equi-probable for finite-input channels, e.g., BSC, BEC, BI-AWGN, or $M$-ary input AWGN
    \item Ex) Gaussian or any other continuous distributions for unconstrained-input (infinite alphabet size) channels with power constraints
    \eitem


\item[iii)] $q_{\calC}(\bfx)$ of (\ref{eq:q_bfx_code_prob}): The code $\calC$ is uniquely mapped to $q_{\calC}(\bfx)$ of (\ref{eq:q_bfx_code_prob}), which can be used for (\ref{eq:P_err^L_q_bfx_init}).
    \bitem \item Ex) This is always uniquely determined by the code \eitem

\item[iv)] $\breve q'(\bfx)$ or $\breve q'(x)$ of (\ref{eq:P_err_L_q_x_final}): For any code including $\calC$, the universal lower bound is obtained by the ensemble average of random codes generated by $\breve q'(\bfx)$, or $\breve q'(x)$ for a single-letter expression. For symmetric DMCs, we have $\breve q'(x) = q_{\rm equ}(x)$.
    \bitem \item Ex) Equi-probable or non-equi-probable for finite-input channels, e.g., BSC, BEC, BI-AWGN, or $M$-ary input AWGN
    \item Ex) Gaussian or any other continuous distributions for unconstrained-input (infinite alphabet size) channels with power constraints
    \eitem
\eitem
Note that the following pairs should be compared:
\bitem
\item Equal a priori probability $\Pr(m)=\frac{1}{M}$ $\Leftrightarrow$ Non-equal a priori probability $\Pr(m)\neq \frac{1}{M}$

\item Finite-input channels (binary-input or $M$-ary input) $\Leftrightarrow$ unconstrained-input (infinite alphabet size) channels with power constraints
\bitem \item Ex) BI-AWGN, $M$-input-AWGN $\Leftrightarrow$ unconstrained-input AWGN with a power constraint \eitem

\item Equi-probable input distribution for finite-input channels $\Leftrightarrow$ Gaussian input distribution for unconstrained-input channels
\bitem \item Ex) $q_{\rm equ}(x)$ $\Leftrightarrow$ $q_{\calN}(x)$ or $q_{\cal CN}(x)$ \eitem

\eitem
\hfill $\Box$

%\newpage
\section{Notation Issue of $q(\bfx)$: Discrete Case}

In \cite{viterbi}, the same notation $q(\bfx)$ is used for achievability \cite[pp. 123--133]{viterbi} and the strong converse \cite[pp. 186--189]{viterbi}. Although the notation is mathematically correct, such usage of the notation is confusing and somewhat misleading, because the meanings are different. As an example, in \cite{viterbi}, for the two expressions of (\ref{eq:P_err_up_q_bfx}) and (\ref{eq:P_err^L_q_bfx_init}), the same notation $q(\bfx)$ is used; and thus, (\ref{eq:P_err_up_q_bfx}) and (\ref{eq:P_err^L_q_bfx_init}) might appear to be equivalent. However, the two forms are {\it not} equivalent because $q(\bfx)$ are defined differently.

To address the issue, in our document, we use different notation: $q(\bfx)$ for  (\ref{eq:P_err_up_q_bfx}) and $q_\calC(\bfx)$ for (\ref{eq:P_err^L_q_bfx_init}). Recall that in (\ref{eq:P_err_up_q_bfx}), $q(\bfx)$ represents the probability distribution that randomly generates codewords of random codes in an ensemble. In (\ref{eq:P_err^L_q_bfx_init}), $q_\calC(\bfx)$ represents the special probability distribution that uniquely specifies a particular code $\calC$. Finally, $q'(\bfx), q'(x)$ and $\breve q'(x) = \arg \min_{q'(x)} P_\err^\low(q'(x))$ are the distributions used to derive a universal bound for any code; in fact, by those probability distributions, an ensemble of random codes is generated and the average over this ensemble serves as the universal lower bound.

Three distributions $q(\bfx)$, $q_\calC(\bfx)$, and $q'(\bfx)$ can be considered as {\it three functions} taking inputs from the same set and giving outputs as probabilities: both takes an input as a vector in the set $\calX^n$; and their outputs are probabilities: \beqa q(\bfx = \bfx_0) &=& {\rm probability}_1, ~~~  \bfx_0 \in \calX^n \\ q_\calC(\bfx = \bfx_0) &=& {\rm probability}_2, ~~~  \bfx_0 \in \calX^n \\ q'(\bfx = \bfx_0) &=& {\rm probability}_3, ~~~  \bfx_0 \in \calX^n \eeqa In particular, $q(\bfx)$ and $q'(\bfx)$ are similar in the sense that both of them generate an ensemble of random codes. However, the nature of $q_\calC(\bfx)$ is very different from the other two.
Because, the three functions are different, and thus, the values of the outputs are generally different: \beq {\rm probability}_1 \neq {\rm probability}_2 \neq {\rm probability}_3  \eeq

In order to clarify this difference among $q(\bfx)$, $q_{\calC}(\bfx)$, and $q'(\bfx)$, we consider an example.



{\it [Example 1]:} Let us consider the case $Q=2$, $n=3$, and $M=2$, where $\calX=A_Q =\{a_1,a_2\}$. Then $\calX^n$ is given by \begin{small} \beqa \calX^n=A_Q^n=\{ (a_1,a_1,a_1), (a_1,a_1,a_2), (a_1,a_2,a_1), (a_1,a_2,a_2), (a_2,a_1,a_1), (a_2,a_1,a_2), (a_2, a_2, a_1), (a_2, a_2, a_2) \} \non \eeqa \end{small} Let $\calC$ denote the code given by \beqa \calC &=& \left[ \begin{array}{c} \bfx_1 \\ \bfx_2 \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1} & x_{1,2} & x_{1,3} \\ x_{2,1} & x_{2,2} & x_{2,3} \end{array} \right]  \eeqa

\subsection{Achievability: Error Upper-Bound when $R< C$}

In order to generate an ensemble of random codes, we suppose that each codeword $\bfx_m$ is drawn from $\calX^n$ by probability distribution $q(\bfx)$ given by
\beq q(\bfx) = q(\bfx_m)= \left\{ \begin{array}{ll} \frac{1}{27}, & {\rm if~} \bfx_m = (a_1,a_1,a_1) \\ \frac{2}{27}, & {\rm if~} \bfx_m \in \{ (a_1,a_1,a_2), (a_1, a_2, a_1), (a_2, a_1, a_1) \} \\ \frac{4}{27}, & {\rm if~} \bfx_m \in \{ (a_1,a_2,a_2), (a_2, a_1, a_2), (a_2, a_2, a_1) \} \\ \frac{8}{27}, & {\rm if~} \bfx_m = (a_2,a_2,a_2) \end{array} \right., ~~~ m=1,2 \label{eq:q_x_m_achievability} \eeq where \beqa \sum_{\bfx_1 \in \calX^n} q(\bfx_1) &= & 1 \\  \sum_{\bfx_2 \in \calX^n} q(\bfx_2) &= & 1  \eeqa
Or, in general, \beq \sum_{\bfx_m \in \calX^n} q(\bfx_m) =1, ~~~{\rm for ~ all~} m=1,2,\cdots,M \eeq

For example, the ensemble of random codes can be generated as follows: \beq \calA_\calC(q(\bfx)) =\{ \calC^{(i)}:i=1,\cdots, 64\} \eeq where \beqa \calC^{(1)} &=& \left[ \begin{array}{c} \bfx_1^{(1)} \\ \bfx_2^{(1)} \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1}^{(1)} & x_{1,2}^{(1)} & x_{1,3}^{(1)}  \\ x_{2,1}^{(1)} & x_{2,2}^{(1)} & x_{2,3}^{(1)} \end{array} \right] = \left[ \begin{array}{ccc} a_1 & a_1 & a_1 \\ a_1 & a_1 & a_1 \end{array} \right] \\ \calC^{(2)} &=& \left[ \begin{array}{c} \bfx_1^{(2)} \\ \bfx_2^{(2)} \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1}^{(2)} & x_{1,2}^{(2)} & x_{1,3}^{(2)}  \\ x_{2,1}^{(2)} & x_{2,2}^{(2)} & x_{2,3}^{(2)} \end{array} \right] = \left[ \begin{array}{ccc} a_1 & a_1 & a_1 \\ a_1 & a_1 & a_2 \end{array} \right] \\ \calC^{(3)} &=& \left[ \begin{array}{c} \bfx_1^{(3)} \\ \bfx_2^{(3)} \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1}^{(3)} & x_{1,2}^{(3)} & x_{1,3}^{(3)}  \\ x_{2,1}^{(3)} & x_{2,2}^{(3)} & x_{2,3}^{(3)} \end{array} \right] = \left[ \begin{array}{ccc} a_1 & a_1 & a_1 \\ a_1 & a_2 & a_1 \end{array} \right] \\ \vdots & & ~~~~~ \vdots \\ \calC^{(64)} &=& \left[ \begin{array}{c} \bfx_1^{(64)} \\ \bfx_2^{(64)} \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1}^{(64)} & x_{1,2}^{(64)} & x_{1,3}^{(64)}  \\ x_{2,1}^{(64)} & x_{2,2}^{(64)} & x_{2,3}^{(64)} \end{array} \right] = \left[ \begin{array}{ccc} a_1 & a_1 & a_1 \\ a_1 & a_2 & a_1 \end{array} \right] \eeqa In the above, $\calC^{(1)}$, $\calC^{(2)}$, $\calC^{(3)}$, $\cdots$, $\calC^{(64)}$ are generated with probability $\frac{1}{27^2}$, $\frac{2}{27^2}$, $\frac{2}{27^2}$, $\cdots$, $\frac{64}{27^2}$, respectively.

When $q(\bfx)$ is given by (\ref{eq:q_x_m_achievability}), it can be written in a product form of $q(x)$ as follows: \beq q(\bfx_m) = q(x_{m,1})q(x_{m,2})q(x_{m,3}), ~~~ m=1,2 \eeq or simply, \beq q(\bfx) = q(x_{1})q(x_{2})q(x_{3}) \eeq
where the input distribution $q(x)$ is given by
\beq q(x) = \left\{ \begin{array}{ll} \frac{1}{3}, & {\rm if~} x = a_1 \\ \frac{2}{3}, & {\rm if~} x = a_2 \end{array} \right. \label{eq:input_dist} \eeq
That is, the ensemble $\calA_\calC(q(\bfx))$ can be created by randomly and independently generating each element of $\calC^{(i)}$ using $q(x)$: $\calA_\calC(q(\bfx)) = \calA_\calC(q(x))$.

{\it Remark 7:} The upper-bound of error probability averaged over the ensemble $\calA_\calC(q(x))$ of all codes in the example can be obtained by $P_\err^\up(q(x))$ of (\ref{eq:P_err_u_any_q_x}) along with $q(x)$ of (\ref{eq:input_dist}). However, in order to show the existence of the {\it best} code(s) (in terms of smallest error probability or largest rate), one must consider the ensemble of random codes with optimal occurrence probability distribution.
For symmetric DMCs, the optimal distribution minimizing the upper-bound of error probability is the equi-probable distribution $q_{\rm equ}(x)=\frac{1}{2}$ if $x=a_1$ or $x=a_2$ \cite[Theorem 7.2]{jelinek}. For the best code(s), we need to generate the ensemble of codes using $q_{\rm equ}(x)$. Then the error upper-bound averaged for the ensemble is given by $P_\err^\up(q_{\rm equ}(x))$. From this, the channel capacity $C$ can be determined: $C$ is the maximum rate $R$ subject to $P_\err^\up(q_{\rm equ}(x))\rightarrow 0 $ as $n \rightarrow \infty$. Finally, note that both $q(x)$ of (\ref{eq:input_dist}) and $q_{\rm equ}(x)$ will generated the same ensemble $\calA_\calC(q(x))$ of codes; however, the occurrence probability distributions are different. \hfill $\Box$

\subsection{Strong Converse: Error Lower-Bound when $R > C$}

In the proof of strong converse, we first consider a specific code. For example, let us consider $\check \calC$: \beqa \check \calC &=& \left[ \begin{array}{c}  \bfx_1(\check \calC) \\ \bfx_2(\check \calC) \end{array} \right] =  \left[ \begin{array}{ccc}  x_{1,1}(\check \calC) &  x_{1,2}(\check \calC) &  x_{1,3}(\check \calC)  \\  x_{2,1}(\check \calC) &  x_{2,2}(\check \calC) &  x_{2,3}(\check \calC) \end{array} \right] = \left[ \begin{array}{ccc} a_1 & a_1 & a_2 \\ a_1 & a_2 & a_2 \end{array} \right] \eeqa
Note that this specific code $\check \calC$ might be one realization of random codes generated by $q(\bfx)$ of (\ref{eq:q_x_m_achievability}), or by $q(x)$ of (\ref{eq:input_dist}), or any other input distribution. Or, for the purpose of strong converse, $\check \calC$ might be simply a deterministic code without defining any input distribution such as (\ref{eq:q_x_m_achievability}) and (\ref{eq:input_dist}) at all.


For this specific code $\check \calC$, under the condition that a priori message probabilities are equal, the special distribution $q_{\check \calC}(\bfx)$ of (\ref{eq:q_bfx_code_prob}) is given by
\beqa q_{\check \calC}(\bfx= \bfx_1(\check \calC)) &=& q_{\check \calC}(\bfx=(a_1,a_1,a_2)) = \frac{1}{2} \\ q_{\check \calC}(\bfx= \bfx_2(\check \calC)) &=& q_{\check \calC}(\bfx=(a_1,a_2,a_2)) = \frac{1}{2} \eeqa
or
\beqa q_{\check \calC}(\bfx) = \left\{ \begin{array}{ll} \frac{1}{2}, & {\rm if~} \bfx = \bfx_1(\check \calC)= (a_1, a_1, a_2) {\rm ~ or~} \bfx=\bfx_2(\check \calC) = (a_1, a_2, a_2) \\ 0, & {\rm otherwise} \end{array} \right. \label{eq:strong_converse_q_bfx} \eeqa
Note that this $q_{\check \calC}(\bfx)$ in (\ref{eq:strong_converse_q_bfx}) is purely determined by the code $\check \calC$, not by the input distribution $q(x)$ in (\ref{eq:input_dist}). Specifically,  a code $\check \calC$ is one-to-one mapped to the distribution $q_{\check \calC}(\bfx)$ in (\ref{eq:strong_converse_q_bfx}): If $q_{\check \calC}(\bfx)$ of (\ref{eq:strong_converse_q_bfx}) is given, the corresponding code is uniquely determined; or, if a code is given, the corresponding distribution $q_{\check \calC}(\bfx)$ in (\ref{eq:strong_converse_q_bfx}) is uniquely determined. Note that it is generally {\it not} possible to write $q_{\check \calC}(\bfx)$ of (\ref{eq:strong_converse_q_bfx}) in the form of $q_{\check \calC}(\bfx)=q_{\check \calC}(x_1)q_{\check \calC}(x_2)q_{\check \calC}(x_3)$.

In general, over all $M$ codewords $\{ \bfx_m (\calC):m=1,\cdots,M\}$ of any arbitrary code $\calC$, we have \beqa \sum_{m=1}^M q_\calC(\bfx_m(\calC)) &=& 1, ~~~~ \forall \calC \eeqa


{\it Remark 8:} The lower-bound of error probability for the specific code $\check \calC$ can be obtained by substituting $q_{\check \calC}(\bfx)$ of (\ref{eq:strong_converse_q_bfx}) into the error expression of (\ref{eq:P_err^L_q_bfx_init}). However, the obtained expression is not in a single letter form. For large $n$, it is an intractable expression, of which computation is infeasible. For $\check \calC$, as in (\ref{eq:P_err_L_q_x_final}), a tractable expression of lower-bound of error probability is obtained by using the worst distribution $\breve q'(x) = \arg \min_{q'(x)}P_\err^\low(q'(x))$. For symmetric DMCs, it can be shown that the worst distribution is equi-probable distribution: $\breve q'(x)=q_{\rm qui}(x)$ (see Appendix A of the report).
Note that the special distribution $q_{\check \calC}(\bfx)$ of (\ref{eq:strong_converse_q_bfx}) used to specify a code $\check \calC$ is generally different from the worst distribution $\breve q'(x)$ used to obtain a (universal) single-letter lower-bound of error probability of the code $\check \calC$. \hfill $\Box$

\section{Notation Issue of $q(\bfx)$: Continuous Case}

{\it [Example 2]:} Let us consider the case $n=3$ and $M=2$, where $\calX=\mathbb{R}$. Then $\calX^n$ is given by $\calX^n =\mathbb{R}^n$. Let $\calC$ denote the code given by \beqa \calC &=& \left[ \begin{array}{c} \bfx_1 \\ \bfx_2 \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1} & x_{1,2} & x_{1,3} \\ x_{2,1} & x_{2,2} & x_{2,3} \end{array} \right]  \eeqa

\subsection{Achievability: Error Upper-Bound when $R< C$}

In order to generate an ensemble of random codes, we suppose that each codeword $\bfx_m$ is drawn from $\calX^n$ by probability distribution $q(\bfx)$ given by $q(\bfx) = \calN(\bfzero,\bfI)$, where \beqa \int_{\bfx_1 \in \calX^n} q(\bfx_1) d\bfx_1 &= & 1 \\  \int_{\bfx_2 \in \calX^n} q(\bfx_2) d \bfx_2 &= & 1  \eeqa
Or, in general, \beq \int_{\bfx_m \in \calX^n} q(\bfx_m) d \bfx_m =1, ~~~{\rm for ~ all~} m=1,2,\cdots,M \eeq

For example, the ensemble of random codes can be generated as follows: \beq \calA_\calC(q(\bfx)) =\{ \calC^{(i)}:i=1,2,\cdots \} \eeq where \beqa \calC^{(1)} &=& \left[ \begin{array}{c} \bfx_1^{(1)} \\ \bfx_2^{(1)} \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1}^{(1)} & x_{1,2}^{(1)} & x_{1,3}^{(1)}  \\ x_{2,1}^{(1)} & x_{2,2}^{(1)} & x_{2,3}^{(1)} \end{array} \right] = \left[ \begin{array}{ccc} 0.1 & -0.4 & 2.1 \\ -3.1 & 0.8 & 0.2 \end{array} \right] \\ \calC^{(2)} &=& \left[ \begin{array}{c} \bfx_1^{(2)} \\ \bfx_2^{(2)} \end{array} \right] =  \left[ \begin{array}{ccc} x_{1,1}^{(2)} & x_{1,2}^{(2)} & x_{1,3}^{(2)}  \\ x_{2,1}^{(2)} & x_{2,2}^{(2)} & x_{2,3}^{(2)} \end{array} \right] = \left[ \begin{array}{ccc} 1.8 & 2.2 & -0.4 \\ 0.9 & 4.1 & 2.2 \end{array} \right] \\  \vdots & & ~~~~~ \vdots \eeqa 

When $q(\bfx)$ is given by $\calN(\bfzero,\bfI)$, it can be written in a product form of $q(x)$ as follows: \beq q(\bfx_m) = q(x_{m,1})q(x_{m,2})q(x_{m,3}), ~~~ m=1,2 \eeq or simply, \beq q(\bfx) = q(x_{1})q(x_{2})q(x_{3}) \eeq
where the input distribution $q(x)$ is given by
\beq q(x) = \calN(0,1) \eeq
That is, the ensemble $\calA_\calC(q(\bfx))$ can be created by randomly and independently generating each element of $\calC^{(i)}$ using $q(x)$: $\calA_\calC(q(\bfx)) = \calA_\calC(q(x))$.

\subsection{Strong Converse: Error Lower-Bound when $R > C$}

In the proof of strong converse, we first consider a specific code. For example, let us consider $\check \calC$: \beqa \check \calC &=& \left[ \begin{array}{c}  \bfx_1(\check \calC) \\ \bfx_2(\check \calC) \end{array} \right] =  \left[ \begin{array}{ccc}  x_{1,1}(\check \calC) &  x_{1,2}(\check \calC) &  x_{1,3}(\check \calC)  \\  x_{2,1}(\check \calC) &  x_{2,2}(\check \calC) &  x_{2,3}(\check \calC) \end{array} \right] = \left[ \begin{array}{ccc} 4.1 & 1.8 & -0.9 \\ 1.2 & 0.2 & 3.1 \end{array} \right] \eeqa
Note that this specific code $\check \calC$ might be one realization of random codes generated by $q(\bfx)=\calN(\bfzero,\bfI)$  or by $q(x)=\calN(0,1)$, or any other input distribution. Or, for the purpose of strong converse, $\check \calC$ might be simply a deterministic code without defining any input distribution such as $q(\bfx)$ and $q(x)$ at all.


For this specific code $\check \calC$, under the condition that a priori message probabilities are equal, the special distribution $q_{\check \calC}(\bfx)$  is given by
\beqa q_{\check \calC}(\bfx= \bfx_1(\check \calC)) &=& q_{\check \calC}(\bfx=(4.1, 1.8, -0.9)) = \frac{1}{2} \delta(\bfx -(4.1, 1.8, -0.9)) \\ q_{\check \calC}(\bfx= \bfx_2(\check \calC)) &=& q_{\check \calC}(\bfx=(1.2, -0.2, 3.1)) = \frac{1}{2} \delta(\bfx-(1.2, -0.2, 3.1))\eeqa
or
\beqa q_{\check \calC}(\bfx) = \left\{ \begin{array}{ll} \frac{1}{2} \delta(\bfx - \bfx(\check \calC)), & {\rm for~} \bfx(\check \calC)= (4.1, 1.8, -0.9) {\rm ~ and ~} \bfx(\check \calC) = (1.2, -0.2, 3.1) \\ 0, & {\rm otherwise} \end{array} \right.  \eeqa

In general, over all $M$ codewords $\{ \bfx_m (\calC):m=1,\cdots,M\}$ of any arbitrary code $\calC$, we have \beqa \sum_{m=1}^M \int_{\bfx_m(\calC) \in \calX^n} q_\calC(\bfx_m(\calC)) d \bfx_m(\calC) &=& 1, ~~~~ \forall \calC \eeqa






















\newpage
\section{Some Discussions}

\bitem

\item {\it Single-letter expression of lower-bound when $R>C$:} As discussed before, for a specific code $\calC$, it is generally not possible to write its lower-bound in a single-letter form. Only when we consider the weakest (most loose) lower-bound, it is given in a single-letter form. Also, this weakest lower-bound is valid for all codes as long as $R> C$.

\item {\it Existence of code for Alice:} Consider the system where Alice transmits data at rate $R$ to Bob in the presence of Eve. Assume $R<C_\bob$ and $R>C_\eve$. For a specific code $\check \calC$, we can write the error lower-bound $P_\err^\low(q_{\check \calC}(\bfx))$ of (\ref{eq:P_err^L_q_bfx_init}) at Eve anyway (although the expression is not in a single-letter form). For $\check \calC$, however, there is no guarantee that the error upper-bound $P_\err^\up(q(x))$ at Bob is valid, because $P_\err^\up(q(x))$ is obtained by averaging over the ensemble and thus valid only for some codes in the ensemble; but, there is no guarantee that $\check \calC$ is such codes.

    On the other hand, the weakest lower-bound $\min_{q(x)} P_\err^\low(q(x))$ is valid for any code in the ensemble. Then it is guaranteed that the error upper-bound $P_\err^\up(q(x))$ at Bob is valid.

\item {\it Determination of Input Distribution at Alice:}
    Let $\breve q(x)$ denote the distribution giving the tightest upper-bound: \beq \breve q(x) = \arg \min_{q(x)} P_\err^\up(q(x)), ~~~~ R<C_\bob \eeq Let $\breve q'(x)$ denote the distribution giving the weakest lower-bound \beq \breve q'(x) = \arg \min_{q'(x)} P_\err^\low(q'(x)), ~~~~ R>C_\eve \eeq
    In order to use the tightest upper-bound we should generate the ensemble using $\breve q(x)$. Note that the weakest lower-bound is still obtained by $\breve q'(x)$.

\eitem






%\newpage
\vspace{1cm}
\bibliographystyle{IEEE}
\begin{thebibliography}{999}

\bibitem{gallager} R. G. Gallager, {\it Information Theory and Reliable Communications.} New York: Wiley, 1968.

\bibitem{Arimoto} S. Arimoto, ``On the converse to the coding theorem for discrete memoryless channels," {\it IEEE Trans. Inf. Theory,} vol. , pp. 357--359, May 1973.

\bibitem{viterbi} A. J. Viterbi and J. K. Omura, {\it Principles of Digital Communication and Coding.}  New York: McGraw-Hill, 1979.

\bibitem{Blahut} R. E. Blahut, {\it Principles and Practice of Information Theory.} Addison-Wesley, 1987.

\bibitem{jelinek} F. Jelinek, {\it Probabilistic Information Theory.} New York: McGraw-Hill, 1968.

\bibitem{cover} T. M. Cover and J. A. Thomas, {\it Elements of Information Theory.} Wiely, 2nd Ed., 2006.

\end{thebibliography}










































































%%%%%
